Beyond Words: Augmenting Discriminative Richness via Diffusions in Unsupervised Prompt Learning

Fine-tuning vision-language models (VLMs) with large amounts of unlabeled data has recently garnered significant interest. However, a key challenge remains the lack of high-quality pseudo-labeled data. Current pseudo-labeling strategies often struggle with mismatches between semantic and visual information, leading to sub-optimal performance of unsupervised prompt learning (UPL) methods. In this paper, we introduce a simple yet effective approach called \textbf{A}ugmenting D\textbf{i}scriminative \textbf{R}ichness via Diffusions (AiR), toward learning a richer discriminating way to represent the class comprehensively and thus facilitate classification. Specifically, our approach includes a pseudo-label generation module that leverages high-fidelity synthetic samples to create an auxiliary classifier, which captures richer visual variation, bridging text-image-pair classification to a more robust image-image-pair classification. Additionally, we exploit the diversity of diffusion-based synthetic samples to enhance prompt learning, providing greater information for semantic-visual alignment. Extensive experiments on five public benchmarks, including RESISC45 and Flowers102, and across three learning paradigms-UL, SSL, and TRZSL-demonstrate that AiR achieves substantial and consistent performance improvements over state-of-the-art unsupervised prompt learning methods.

==> CVPR2025_v2/Figures/beta.tex <==
\begin{figure}
\centering

\includegraphics[width=.9\linewidth]{Images/beta.png}
% \vspace{-5pt}
\caption{
Comparison of top-1 test accuracy ($\%$) of pseudo labels with different hyper-parameters $\beta$.
}
% \vspace{-20pt}
\label{fig:beta}
\end{figure}

==> CVPR2025_v2/Figures/cam.tex <==
\begin{figure}
\centering

\includegraphics[width=.9\linewidth]{Images/cam_v2.pdf}
% \vspace{-5pt}
\caption{
Visualization of the activation regions for the text classifier and synthetic-sample-based auxiliary classifier using CAM. 
`T $\&$ S' represents the activation after merging the outputs of both classifiers.
}
\vspace{-15pt}
\label{fig:cam}
\end{figure}

==> CVPR2025_v2/Figures/intro.tex <==
\begin{figure}[!tb]
\centering
\includegraphics[width=1\linewidth]{Images/intro_v2.pdf}
\caption{
Left: Confusion matrix for ground truth labels $vs.$ text classifier predictions on the Flowers102 dataset, highlighting persistent generation of incorrect pseudo-labels.
Right: An example of misclassification in Flowers102, where ``Thorn apple" is misidentified as ``Giant white arum lily" due to its white petals resembling the latter’s semantic information. This misclassification can be alleviated by jointly considering text and image predictions.
}
\vspace{-20pt}
\label{fig:intro}
\end{figure}

==> CVPR2025_v2/Figures/lamada.tex <==
\begin{figure}
\centering

\includegraphics[width=.9\linewidth]{Images/lambda.png}
% \vspace{-5pt}
\caption{
Comparison of top-1 test accuracy ($\%$) of pseudo labels with different hyper-parameters $\lambda$. 
% `Ours' denotes the use of our approach AiR, while `CLIP' indicates the use of only CLIP's text encoder.
}
% \vspace{-20pt}
\label{fig:lamada}
\end{figure}

==> CVPR2025_v2/Figures/lnl.tex <==
\begin{figure}
\centering

\includegraphics[width=.85\linewidth]{Images/lnl.png}
% \vspace{-5pt}
\caption{
Comparison results of top-1 test accuracy ($\%$) on unsupervised learning with or without LoRA fine-tuning.
Note that `w/o' denotes the synthetic sample generated without LoRA.
}
% \vspace{-5pt}
\label{fig:lnl}
\end{figure}

==> CVPR2025_v2/Figures/method.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=0.75\linewidth]{Images/method_v9.pdf}
\caption{{
Overview of our proposed AiR, which consists of ACG (Auxiliary Classifier Generation) Module and PLG (Pseudo Label Generation) Module.
ACG generates synthetic samples using the LoRA fine-tuned SD model and selects the representative samples by cosine similarity to build auxiliary classifier. PLG generates  pseudo-labels by fusing the predictions of the auxiliary classifier built on synthetic images and the text classifier.
The overall loss for training prompt consists of the classification loss of real images with pseudo-labels $\mathcal{L}_{r}$ and classification loss of synthetic images with corresponding categories $\mathcal{L}_{s}$, where ours can learn visual and textual prompt.}
}
\vspace{-10pt}
\label{fig:method}
\end{figure*}

==> CVPR2025_v2/Figures/num.tex <==
\begin{figure}
\centering

\includegraphics[width=.9\linewidth]{Images/num.png}
% \vspace{-5pt}
\caption{
Comparison of top-1 test accuracy ($\%$) across varying numbers of synthetic samples in unsupervised learning on the RESISC45 and EuroSAT datasets.
% The bubble sizes represent the proportion of synthetic samples to real samples.
}
\vspace{-10pt}
\label{fig:nu}
\end{figure}

==> CVPR2025_v2/Figures/only.tex <==
\begin{figure}
\centering

\includegraphics[width=.85\linewidth]{Images/only.png}
% \vspace{-5pt}
\caption{
Comparison of top-1 test accuracy ($\%$) in unsupervised learning, with or without the inclusion of real samples in the loss functions. `S$\&$R' denotes the use of both synthetic and real samples for loss calculation, while `S' indicates the use of only synthetic samples.
}
% \vspace{-5pt}
\label{fig:on}
\end{figure}

==> CVPR2025_v2/Figures/pla.tex <==
\begin{figure}
\centering

\includegraphics[width=.8\linewidth]{Images/pla.png}
% \vspace{-5pt}
\caption{
Comparison of top-1 test accuracy ($\%$) of pseudo labels in unsupervised learning. 
`Ours' denotes the use of our approach AiR, while `CLIP' indicates the use of CLIP's text encoder.
}
\vspace{-15pt}
\label{fig:pla}
\end{figure}

==> CVPR2025_v2/Figures/plaa.tex <==
\begin{figure}
\centering

\includegraphics[width=.9\linewidth]{Images/CPL_VS_OURS.png}
% \vspace{-5pt}
\caption{
Comparison of top-1 test accuracy ($\%$) of pseudo labels during different training iterations.
}
% \vspace{-15pt}
\label{fig:plaa}
\end{figure}

==> CVPR2025_v2/Figures/sum.tex <==
\begin{figure}
\centering
\vspace{-15pt}
\includegraphics[width=1\linewidth]{Images/sum_v3.pdf}
% \vspace{-20pt}
% \caption{Additional results.
% }
\vspace{-35pt}
\label{fig:sum}
\end{figure}


% Experiments:(a) for \noindent\textbf{\textit{Major Q1}} \textbf{\textit{\textcolor{red}{vVNT}}} and \noindent\textbf{\textit{Q4}} \textbf{\textit{\textcolor{blue}{Lp4P}}}, (b) for \noindent\textbf{\textit{Q1}} \textbf{\textit{\textcolor{cyan}{7Tnt}}}, (c) for \noindent\textbf{\textit{Q5}} \textbf{\textit{\textcolor{blue}{Lp4P}}} and (d) for \noindent\textbf{\textit{Minor Q3}} \textbf{\textit{\textcolor{red}{vVNT}}}.   

==> CVPR2025_v2/Figures/syt.tex <==
\begin{figure}
\centering

\includegraphics[width=.9\linewidth]{Images/syt_v2.pdf}
% \vspace{-5pt}
\caption{
Visualization of real images and synthetic images generated by the SD model, with and without fine-tuning via LoRA.
}
\vspace{-15pt}
\label{fig:syn}
\end{figure}

==> CVPR2025_v2/Figures/tsne.tex <==
\begin{figure}
\centering

\includegraphics[width=.9\linewidth]{Images/tsne_v4.pdf}
% \vspace{-5pt}
\caption{
Visualization of the spatial distribution of synthetic image, text, and sample embeddings
with t-SNE, respectively.
Circular dots in different colors represent distinct image classes in Flowers102, triangles indicate text embeddings for each class, squares represent synthetic image embeddings, and pentagrams denote the embeddings after fusing text and synthetic image embeddings.
}
\vspace{-20pt}
\label{fig:tsne}
\end{figure}

==> CVPR2025_v2/Figures/tsnee.tex <==
\begin{figure}
\centering

\includegraphics[width=.9\linewidth]{Images/tsne_v3_res_v2.pdf}
% \vspace{-5pt}
\caption{
Visualization of the spatial distribution of synthetic image, text, and sample embeddings
with t-SNE in RESISC45 dataset.
}
% \vspace{-20pt}
\label{fig:tsres}
\end{figure}

==> CVPR2025_v2/Figures/tsneee.tex <==
\begin{figure}
\centering

\includegraphics[width=.9\linewidth]{Images/tsne_v3_dtd_v2.pdf}
% \vspace{-5pt}
\caption{
Visualization of the spatial distribution of synthetic image, text, and sample embeddings
with t-SNE in DTD dataset.
}
% \vspace{-20pt}
\label{fig:tsdtd}
\end{figure}

==> CVPR2025_v2/Sections/0_abstract.tex <==
\begin{abstract}
Fine-tuning vision-language models (VLMs) with large amounts of unlabeled data has recently garnered significant interest. 
However, a key challenge remains the lack of high-quality pseudo-labeled data. 
Current pseudo-labeling strategies often struggle with mismatches between semantic and visual information, leading to sub-optimal performance of unsupervised prompt learning (UPL) methods.
In this paper, we introduce a simple yet effective approach called \textbf{A}ugmenting D\textbf{i}scriminative \textbf{R}ichness via Diffusions (AiR), toward learning a richer discriminating way to represent the class comprehensively and thus facilitate classification.
Specifically, our approach includes a pseudo-label generation module that leverages high-fidelity synthetic samples to create an auxiliary classifier, which captures richer visual variation, bridging text-image-pair classification to a more robust image-image-pair classification. 
Additionally, we exploit the diversity of diffusion-based synthetic samples to enhance prompt learning, providing greater information for semantic-visual alignment.
Extensive experiments on five public benchmarks, including RESISC45 and Flowers102, and across three learning paradigms-UL, SSL, and TRZSL-demonstrate that AiR achieves substantial and consistent performance improvements over state-of-the-art unsupervised prompt learning methods.
\href{https://github.com/Hrren/Beyond-Words}{Code} is available.

\end{abstract}

==> CVPR2025_v2/Sections/1_Introduction.tex <==
\section{Introduction}
\label{sec:intro}
 % !!!!! Key word: Visual Perception, requiring a high level of visual comprehension, high-fidelity
% Large pre-trained vision-language models (VLMs)\cite{radford2021learning, yuan2021florence, jia2021scaling} have demonstrated remarkable performance in open-world visual concept learning without
% task-specific training but still requires adaptation for optimal performance. 
% Prompt tuning \cite{ge2023domain, jia2022visual} provides an efficient approach to boost VLMs' discriminative accuracy on downstream tasks by learning inputs to the model. 
Large pre-trained vision-language models (VLMs)~\cite{radford2021learning, yuan2021florence, jia2021scaling} have achieved impressive performance in open-world visual concept learning without requiring task-specific training; however, they still benefit from adaptation for optimal results.
Prompt tuning \cite{ge2023domain, jia2022visual, 10740179, 10342801} offers an efficient strategy to enhance VLMs' discriminative accuracy on downstream tasks by learning inputs to the model.

% While learning prompts yield significant improvements, the substantial labeled data is still necessary to improve the performance of VLMs for adaptation on various downstream tasks. This requirement for adaptation would cause considerable labeling costs, as labeled data is hard to obtain\cite{tanwisuth2023pouf, zhou2022learning, zhou2022conditional}. To this end, unsupervised prompt learning (UPL)\cite{huang2022unsupervised, menghini2023enhancing, lai2023padclip, shu2022test} is proposed to learn adaptive prompts with pseudo labels generated by the inherent zero-shot ability of VLMs, which becomes an effective approach for exploiting unlabeled data. 
% For pseudo-labeling, conventional methods \cite{huang2022unsupervised} first input the prompt with words of the class name of the current dataset to VLMS' text encoder to form a text classifier. 
% Then assign image embedding of unlabeled data to these words' text classifier with high-confidence predictions to generate pseudo label. 
% Some other approaches\cite{menghini2023enhancing, zhang2024candidate} get multiple candidate pseudo-labels by expanding the confidence threshold to alleviate the class imbalance problem or optimize the model by using different numbers of pseudo-label samples at different stages of training.
% \gdd{Although these methods design different strategies to filter pseudo-labels or learn the prompt, most of them depend on the pseudo labels given by the above text classifier.}
% Therefore, the quality of the pseudo-labels is particularly important.
While prompt learning can yield notable improvements, a large amount of labeled data is still required to enhance VLMs' performance across diverse downstream tasks. 
This adaptation requirement leads to considerable labeling costs, as labeled data is hard to obtain \cite{tanwisuth2023pouf, zhou2022learning, jia2024revealing, zhou2022conditional}. 
To address this, unsupervised prompt learning (UPL) \cite{huang2022unsupervised, menghini2023enhancing, lai2023padclip, shu2022test} has been introduced, leveraging the zero-shot capabilities of VLMs to generate pseudo labels, enabling effective use of unlabeled data.
For pseudo-labeling, traditional methods \cite{huang2022unsupervised} typically form a text classifier by inputting prompts with class names into the VLMs' text encoder. 
Then, image embeddings of unlabeled data are matched to these class-based text classifiers, assigning pseudo-labels to images with high-confidence predictions. 
Some other approaches \cite{menghini2023enhancing, zhang2024candidate} generate multiple candidate pseudo-labels by adjusting confidence thresholds or optimize the model with different numbers of pseudo-labeled samples at various training stages. 
While these methods apply distinct strategies for filtering pseudo-labels or refining prompts, most ultimately rely on pseudo-labels produced by text classifiers, making the quality of these pseudo-labels critically important.
% Thus, the performance of the existing methods heavily relies on the accuracy of the generated pseudo labels.


\input{Figures/intro}

% Thus, the performance of the existing methods heavily relies on the accuracy of the generated pseudo labels.
\gdd{In this work, we aim to improve the pseudo label quality in UPL, which can thus be easily combined with other UPL methods. Here, we first explore conduct a pilot experiment to empirically demonstrate the deficiency of text classifiers.  }
% To illustrate this issue, we conducted a pilot experiment to empirically demonstrate the deficiency of text classifiers.
Specifically, we leverage the text encoder of CLIP~\cite{radford2021learning} to generate pseudo labels on the Flowers102 dataset~\cite{nilsback2008automated} and subsequently calculated the confusion matrix between the ground-truth labels and predicted class labels.
The results, as shown in Fig.~\ref{fig:intro}, reveal that a substantial number of samples are incorrectly predicted, $e.g.$, most ``Thorn apple'' flowers are misclassified as ``Giant white arum lily'', ``Tree mallow'' is misclassified as ``Mexican petunia''.
Why this happened? The discrimination of unlabeled images heavily relies on the precision of text classifiers, which are constructed using the words of prompt with category label names.
% Through further careful observation, we find that most of these misclassified samples are discriminated into categories that are more descriptive of one of their attributes.
% The Thorn apple flower has a trumpet-shaped structure, shades of white color, and a wavy edge.
% That is to say, one class can be described by many intrinsic characteristics and even extrinsic context relations. 
\gdd{However, when only using the text of ``a photo of a + class name'' to describe the image, using ``Giant white arum lily'' as the class name is even closer in semantics to the given image than ``Thorn apple''.
Because the Thorn apple flower appears to be a shade of white but the word ``Thorn apple'' does not express that, resulting in the misclassified samples. It motivates us to learn a richer discriminating way to represent the class comprehensively and thus facilitate classification. Since an image has rich information, we consider a novel solution: in addition to the text classifier built on the short text description, can we design another auxiliary classifier based on the most representative images for each category? However, this solution is problematic since we do not know the ground-truth label of each training image in the unsupervised prompt learning task, making it a dead-end loop.}

% However, the word ``Sweet-pea'' does not accurately describe these properties; instead, ``Purple-coneflower'' is closer to this description, which in turn causes a large number of samples to be misclassified. It motivates us to learn a richer discriminating way to represent the class comprehensively and thus facilitate classification.

% \gdd{The most natural solution is to directly get the most representative images for each category and respectively match each test sample with the ground-truth samples in image modality. In other words, the classification of unlabeled images is expanded from text-image pairs used by a text classifier, which relies solely on semantic information, to image-image pairs used by an image classifier, which provides abundant visual information. However, this solution is problematic since it is the lack of labels that leads to inaccurate unsupervised learning of downstream tasks that require richer discriminative information, and now the need for ground-truth samples for reference, which turns into a dead-end loop.}


% The most natural solution is to directly get the most representative images for each category and respectively match each test sample with the ground-truth samples in image modality.
% In other words, the classification of unlabeled images is expanded from text-image pairs used by a text classifier, which relies solely on semantic information, to image-image pairs used by an image classifier, which provides abundant visual information. However, this solution is problematic since it is the lack of labels that leads to inaccurate unsupervised learning of downstream tasks that require richer discriminative information, and now the need for ground-truth samples for reference, which turns into a dead-end loop.



\gdd{To address the above problem, in this paper, we draw inspiration from the image generation literature. Recent advancements in image generation have made it possible to generate fidelity and diverse images with only text word descriptions, such as Stable Diffusion \cite{rombach2021highresolution}. It is effective in generating diverse images with richer visual appearance variation while preserving the key semantics. Surprisingly, we find that this text-to-image generation model can be naturally utilized to generate the synthetic representative images for each class in UPL tasks only with the text descriptions on the class names. Therefore, we propose Beyond Words: \textbf{A}ugmenting D\textbf{i}scriminative \textbf{R}ichness via Diffusions, a new framework \textbf{AiR} which applies diffusion models to generate synthetic images, which serve as a bridge from text-image-pair to image-image-pair classification, as a way to discriminate the unlabeled images. In our AiR framework, we adopt Stable Diffusion \cite{rombach2021highresolution} to generate discriminative richness, where we fine-tune the Stable Diffusion model with LoRA \cite{hu2022lora} by means of pseudo-labeled samples with high confidence to ensure prediction fidelity. Then, we introduce cosine similarity-based filtration to select the most representative synthetic image of each class generated by fine-tuned Diffusion, which is used to build the auxiliary classifier from the view of the image. Combining the predictions of the original text classifier and the auxiliary classifier, we can endow the training images with more accurate pseudo labels, improving the UPL performance. Besides, the diffusion-based synthetic samples can also be utilized to learn the prompt. Notably, our proposed AiR only needs to know the dataset name and class name of downstream tasks, which can be seamlessly integrated into most UPL methods}. Experimental results show that AiR achieves a notable improvement in classification accuracy by an average of 2.6\% in comparison to the state-of-the-art UPL method. To sum up, our contributions can be included:
\begin{itemize}
    \item We highlight that relying solely on the text classifier to generate pseudo labels in UPL is inadequate and propose a richer discriminating way to represent the class comprehensively and thus facilitate classification.
    \item We present a novel approach AiR: \textbf{A}ugmenting D\textbf{i}scriminative \textbf{R}ichness via Diffusions. 
    This method leverages the diversity and fidelity of synthetic samples to build an auxiliary classifier that captures richer variations in visual appearance while preserving essential semantics, bridging text-image-pair classification to image-image-pair classification.
    \item Our AiR demonstrates substantial improvement across three distinct unsupervised paradigms and five widely-used datasets, significantly outperforming the current state-of-the-art UPL method by an average margin of over 2.6\%.
\end{itemize}

\input{Figures/method}

% Therefore, we propose Beyond Words: \textbf{A}ugmenting D\textbf{i}scriminative \textbf{R}ichness via Diffusions, a new framework \textbf{AiR} which applies diffusion models to generate synthetic images, which serve as a bridge from text-image-pair to image-image-pair classification, as a way to discriminate the unlabeled images.
% In our AiR framework, we adopt Stable Diffusion [] to generate discriminative richness from the view of image.
% Stable Diffusion is a text-to-image generation model which synthesizes an image based on the word's text feature.
% The diffusion-based augmentation is effective in generating diverse images with richer visual appearance variation while preserving the key semantics.
% Furthermore, we leverage both the real samples in training data and diffusion-based synthetic samples for improving UPL performance.
% To ensure prediction fidelity, we finetune the Stable Diffusion model with LoRA by means of pseudo-labeled samples with high confidence, and we also introduce cosine similarity-based filtration to remove spurious augmentations.
% Moreover, AiR only needs to know what the dataset names are for downstream tasks and can be seamlessly integrated into arbitrary CLIP architectures.
% Experimental results show that AiR achieves a notable improvement in classification accuracy by an average of 3.13\% in comparison to the state-of-the-art UPL method. 
% To sum up, our contributions are as follows:


==> CVPR2025_v2/Sections/2_related.tex <==
\section{Related Work}
\label{sec: rw}

\subsection{Prompt Learning}
\label{ssec:pl}
Prompt learning is a technique that enhances the practical application of large pre-trained models like CLIP \cite{radford2021learning} and GPT \cite{brown2020language, radford2019language} by enabling improved performance across various downstream tasks through tailored text or visual prompts. 
For instance, CoOp~\cite{zhou2022learning} optimizes continuous prompt vectors instead of relying on discrete ones, thereby avoiding the suboptimal performance caused by hand-designed prompts. 
CoCoOp~\cite{zhou2022conditional} addresses CoOp's generalization challenges by incorporating Meta-Net, which balances performance between base and novel classes.
When only unlabeled data is available, some work is dedicated to unsupervised learning to accomplish prompt learning.
UPL~\cite{huang2022unsupervised} using CLIP’s~\cite{radford2021learning} zero-shot capabilities, followed by confidence refinement to generate pseudo-labels with higher confidence for unsupervised learning.
IFPL and GRIP~\cite{menghini2023enhancing}, proposed `Iterative Refinement of Few-pseudo labels' and `Grow and Refine Iteratively Pseudolabels' respectively, in terms of how to utilize pseudo-labelled samples.
To alleviate the issue of hard pseudo labels, CPL \cite{zhang2024candidate}, proposes a
Candidate Pseudolabel Learning method, which progressively generates refined candidate pseudo labels by both intra- and inter-instance label selection. \gdd{Different from these pseudo-labeling \cite{menghini2023enhancing, zhang2024candidate, huang2022unsupervised} approaches, which typically rely on text classifiers to generate pseudo labels. 
We propose the AiR framework, which uses synthetic images as a bridge to expand text-image-pair classification with image-image-pair classification, further improving the model's discriminative performance from a richer visual perspective.}
% \subsection{Synthetic Image Generation}
% \label{ssec:sig}
% The suite of image generation models is growing, including Variational Auto-Encoders, GANs and Diffusion Models.
% With their recent popularity, diffusion models such as Stable Diffusion, SDXL, DALL-E, Imagen, GLIDE, and Wuerstchen have revolutionized text-to-image generation. 
% A pool of research has blossomed in its wake, exploring downstream applications; namely: can models be trained on synthetic data? 
% Some works augmented real datasets with synthetic images.
% Others focused on pre-training on large amounts of synthetic data, followed by
% fine-tuning on a limited number of real images. 
% Similarly, several works evaluated the effectiveness of training on entirely synthetic datasets.
\subsection{Training with Synthetic Data}
The diffusion model (DM) has shown significant effectiveness in various synthetic tasks, including image \cite{ho2020denoising, song2020denoising}, video \cite{bar2022text2live}, audio \cite{kong2020diffwave}, and text \cite{li2022diffusion}.
Concurrently, DM has made notable advancements in image manipulation and restoration tasks, such as image editing \cite{avrahami2022blended}, inpainting \cite{lugmayr2022repaint}, and deblurring \cite{whang2022deblurring}.
In the field of prompt learning, exploration has also been undertaken. 
For example, DiffTPT \cite{feng2023diverse} generates diverse augmented images with diffusion models while faithfully preserving the key semantics.
DataDream \cite{kim2024datadream}, a novel few-shot method that adapts Stable Diffusion to generate better in-distribution images for downstream training and is also proven effective in the field of prompt learning.
However, most of the aforementioned methods primarily focus on leveraging diffusion models (DM) for data augmentation or generating more realistic images, without employing DM as a bridge to connect the unsupervised text modality with the image modality. 
Furthermore, the application of DM within unsupervised prompt learning (UPL) remains largely unexplored.


==> CVPR2025_v2/Sections/3_method.tex <==
\section{Method}
\label{sec:method}


\subsection{Preliminaries}
\label{ssec:pre}
\noindent\textbf{Revisiting Unsupervised Prompt Tuning.}
We provide a brief introduction to the prevailing unsupervised prompt learning (UPL) method.
In the UPL setting, we have access only to unlabeled data $X_U = \{x_i\}_{i=1}^N$ composed of $N$ instances with target classes name $\{y_1, ..., y_C \}$.
% the goal is to assign labels to data points in which the model is most confident.
% Suppose a VLM with learnable prompt parameters $t$, where $t$ is typically ``a photo of a" in the CLIP zero-shot setting. 
\gdd{Suppose a VLM with learnable prompt parameters $t$. 
 Besides, in the CLIP zero-shot setting, ``a photo of a" is a usually used prompt, denoted as $t_{zs}$.} Each class name $\{y_c\}_{c=1}^C$ is concatenated with a text prompt to formulate a text input ``a photo of a [CLS]", which is represented as $w_{c}=\{\rr{t_{zs}}, y_c\}$ and can be fed into the text encoder $G$ in VLM to yield a text embedding $g_c = G(w_{c})$. Concurrently, given an instance $x$ in $X_U$, we can embed it with image encoder $F$ of CLIP to produce a visual embedding $f = F(x)$.
The prediction probabilities over classes are given as follows:
\begin{equation}
p_c = \frac{\text{exp}(\text{sim}({f}, {g}_c) / \tau)}{\sum_{c^{\prime}=1}^C \text{exp}(\text{sim}({f}, {g}_{c^{\prime}}) / \tau)},
\label{eq:zc}
\end{equation}
where $\tau$ represents the temperature coefficient.
Besides, $\text{sim}(\cdot)$ refers to a metric function for measuring the similarity between the input image and the text, which is realized with cosine similarity.
Mainstream UPL methods such as FPL \cite{huang2022unsupervised}, GRIP \cite{menghini2023enhancing} employ CLIP's zero-shot capability to assign a pseudo-label $\tilde{y}$ to each sample $x$ as follows:
% Then We can easily identify the prediction pseudo label  $\tilde{y}$ by:
\begin{equation}
\tilde{y} = \underset{c}{\text{argmax}}p_c,
\label{eq:pl}
\end{equation}
typically, one can use a top-$K$ pseudo labeling approach, where the top-$K$ most confident examples per class are used as pseudo-labeled data.
Then, the prompts $t$ can be optimized via back-propagating the following loss:
\begin{equation}
\underset{t}{\text{min}}\mathcal{L}_{ce} = \underset{t}{\text{min}}\mathbb{E}_{({x},\tilde{y})} \left[-\text{log}p(\tilde{y}|{x})\right].
\label{eq:ce}
\end{equation}
However, due to the limited expressive power of purely semantic information, the accuracy of pseudo-labels generated by text-only classifiers remains sub-optimal. 


\subsection{Overview}
This work aims to improve the pseudo-labeling accuracy in UPL from a novel view. Specifically, we extend text-image-pair classification to image-image-pair classification by generating synthetic samples for each category, enhancing the classifier’s visual perception with the Diffusion Model (DM), which serves as a bridge. The overall workflow of our method can be divided into three steps: 
\textcircled{1} 
Finetune DM with LoRA.
Considering the need to ensure the diversity of the synthetic samples while making the synthetic samples more consistent with the domain distribution of the current downstream dataset, we use the LoRA strategy to finetune the DM(see Sec. \ref{ssec:fd}).
\textcircled{2} 
\textbf{ACG} (Auxiliary Classifier Generation) Module: After finetuning with LoRA, we generate synthetic images through the DM with descriptions of the dataset and class name.
Then, we obtain the auxiliary classifier with cosine similarity and select a representative sample for each class.
(see Sec. \ref{ssec:sd}).
\textcircled{3}
\textbf{PLG} (Pseudo Label Generation) Module: Based on the synthetic image, we expand text-image-pair prediction with image-image-pair prediction, further improving the model's discriminative performance from a richer visual perspective and obtaining a more comprehensive pseudo label (see Sec. \ref{ssec:lw}). 
% \gdd{Finally we iterate the preceding steps (which step needs to be iterated? steps 1-3 or steps 2-3 or step3?)} until the model’s parameters are optimized for downstream tasks.
% This iterative process facilitates the progressive refinement
% and optimization of pseudolabels.

\subsection{Finetune DM with LoRA}
\label{ssec:fd}
% Albeit diffusion-based models are effective in generating diverse images,
While the DM can generate a diverse range of images through text-to-image generation, these images do not always align with the dataset of the downstream task. 
This may introduce spurious classes and style mismatches, leading to domain inconsistency and degraded prompt tuning performance.
% DM is able to generate a diversity of different images by means of text-to-image generation, however, these images do not always match the dataset of the downstream task,
% some spurious classes and mismatched styles may be introduced, resulting in domain inconsistency and collapsing prompt tuning performance.
Thus, it is necessary to balance the augmented images' data diversity and domain consistency.
The most straightforward approach would be to fine-tune the DM using labeled datasets from downstream tasks; however, this method is computationally expensive, and labeled data is unavailable. \gdd{To this end, we adopt CLIP's zero-shot generated pseudo-labeled data $\{x, \tilde{y}\}$ in Sec.~\ref{ssec:pre} to fine-tune the DM with LoRA \cite{hu2022lora}, where we employ Stable Diffusion (SD) and the details about the LoRA is deferred to Appendix.}
The original SD model parameters $\theta$ are kept frozen and only the LoRA weights $\delta$ are trained with the objective function:
\begin{equation}
\underset{\delta}{\text{min}}\mathcal{L}_{lora} \!=\! \underset{\delta}{\text{min}}\mathbb{E}_{\rr{({x},\tilde{y})}, \epsilon \sim \mathcal{N}(0, 1)}([||\epsilon \!-\!\epsilon_{\theta, \delta}(x,t_{data},\tilde{y})||_2^2],
\label{eq:lora}
\end{equation}
where $\epsilon \sim \mathcal{N}(0, 1)$ denotes the sampled noise, $\epsilon_{\theta, \delta}(\cdot)$ denotes the noise generated by SD model. \gdd{In addition to the training image $x$ and its pseudo-label $\tilde{y}$ generated by zero-shot CLIP, the description of the dataset $t_{data}$ is also the input of the SD model, to ensure that the generation of samples is more in line with the current dataset. Taking the Flowers102 dataset as the example, $t_{data}$ is ``Flowers:'' and $\tilde{y}$ may be ``Thorn apple'' or any class else.} In this way, we ensure both the diversity of the synthesized samples and domain consistency to the current dataset domain. For subsequent synthetic images, we used the LoRA-updated SD model for generation.


% \subsection{SD-based Synthetic Image Generation}
\subsection{ACG Module}
\label{ssec:sd}
After fine-tuning with LoRA, SD is presented to generate diverse and domain-consistency data.
% In order to ensure that the generation of samples is more in line with the current dataset, as shown in Fig\ref{fig:method}, we generate synthetic images by using a description of the dataset $t_d$, and the class name $y_c$ for which images we want.
% $e.g.$ for the RESISC45 dataset, $t_d$ is `Remote Sensing Image Scene: ', $y_c$ is `airplane' or `airport' or any class else.
% given natural language descriptions of current dataset $t_d$ and class name $y_c$,
For each class in the UPL task, we can generate synthetic data with the SD model $S(\cdot)$ as:
\begin{equation}
\rr{\hat{X}_{c}^M = S(\{t_{data}, y_c\}, \epsilon)},
\label{eq:ds}
\end{equation}
where $\hat{X}_{c}^M = \{\hat{x}_{c}^i\}_{i=1}^M$ represents the generated synthetic images of class $y_c$ and $M$ denotes the number of images generated for each class. 
% Then We can use these generated images to prepare for the next expansions of text-image classification with image-image classification.
Considering the synthetic image needs to be used as the auxiliary classifier, it is essential to select the representative sample from $\hat{X}_c^M$ that best aligns with the semantic information of the current category. Following \cite{feng2023diverse}, we compute the cosine similarity between the zero-shot CLIP text embedding $g_c$ and each synthetic image in $\hat{X}_c^M$. Using Eq. \ref{eq:zc}, we then select the synthetic sample with the highest confidence $p_c$ for each class $c$ and achieve the following synthetic dataset:
\begin{equation}
\hat{X}^* = \{\hat{x}_1^*, \hat{x}_2^*, ..., \hat{x}_C^* \}.
\label{eq:xf}
\end{equation}
\gdd{We now build the bridge between the text class name and the representative synthetic dataset. Here, $\hat{x}_c^*$ is the most representative synthetic image for the $c$-th class and it contains the ample visual perceptual discrimination information, exactly what the textual class name used in zero-shot CLIP lacks. Therefore, it is natural to extract the visual embedding of $\hat{X}^*$ with the vision encoder $F$ and build the auxiliary classifier based on the visual prototypes.}

% Although the synthetic images $\hat{X}_c$ generated by the SD model contain ample visual perceptual information, to build our auxiliary classifier


% Taking these synthetic images into account, the discrimination of an unlabeled image can not only in terms of the text-image-pair: semantic information $\{t, y_c\}$, but also in terms of the image-image-pair: synthetic image $\hat{X}=\{\hat{x}_i^1, \hat{x}_i^2, ..., \hat{x}_i^C\}_{i=1}^N$.
% Albeit diffusion-based models are effective in generating diverse images, some spurious classes and mismatched styles may be introduced, resulting in domain-inconsistency and collapsing prompt tuning performance.
% Thus, it is necessary to balance the augmented images' data diversity and domain consistency.
% To tackle this issue, we introduce $LoRA$ with pseudo-labeled data $\{x, \tilde{y}\}$ to fine-tune the diffusion model. 
% The original stable diffusion model parameters are kept frozen and only the $LoRA$ weights $\sigma$ are trained with the objective function:
% \begin{equation}
% \underset{\sigma}{\text{min}}\mathcal{L}_{lora} = \underset{\sigma}{\text{min}}\mathbb{E}_{({x}_i,\tilde{y}_i), \epsilon \sim \mathcal{N}(0, 1)}([||\epsilon-\epsilon_{\theta, \sigma}(x,\tilde{y})||_2^2],
% \label{eq:lora}
% \end{equation}
% where the $\epsilon_{\theta, \sigma}(\cdot)$ denotes the noise generated by stable diffusion model with image-text-pair $\{x, \tilde{y}\}$.
% In this way, we ensure both the diversity of the synthesized samples and domain consistency to the current dataset domain.

% \subsection{Learning with Synthetic Image}
\subsection{PLG Module \& Learning with Synthetic Image}
\label{ssec:lw}
% Taking the synthetic image into account, the discrimination of an unlabeled image can not only in terms of the text-image-pair: semantic information $\{t, y_c\}$, but also in terms of the image-image-pair: synthetic image $\hat{X}=\{\hat{x}_i^1, \hat{x}_i^2, ..., \hat{x}_i^C\}_{i=1}^N$.
% The synthetic images generated by the SD model already contain sufficient visual perceptual information, but considering that the quality of the synthetic images varies, and the use of synthetic images as classifiers, it is necessary to find the sample that best matches the semantic information of the current category from m samples.

% Considering that the $M$ images in each category may not all exactly match the corresponding category $y_c$, we follow\cite{}, which performs fine-grained filtering of the samples in $\hat{X}$ to find the image samples that best represent the current category as an additional image classifier.
% To tackle this, following \cite{feng2023diverse}, we calculate the cosine similarity between the zero-shot CLIP's text embedding $g_c$ with each synthetic image in $\hat{X}_c$, then, by using Eq.\ref{eq:zc}, we select the largest confidence $p_c$ corresponding to the synthetic sample as our synthetic image classifier as:
% The synthetic images $\hat{X}_c = \{\hat{x}_i\}_{i=1}^M$ generated by the SD model contain ample visual perceptual information. 
% However, given the variable quality of these images and their role as classifiers, it is essential to select the sample that best aligns with the semantic information of the current category from among the $M$ samples. To address this, following \cite{feng2023diverse}, we compute the cosine similarity between the zero-shot CLIP text embedding $g_c$ and each synthetic image in $\hat{X}_c$.
% Using Eq.\ref{eq:zc}, we then select the synthetic sample with the highest confidence $p_c$ as our synthetic image classifier, defined as:
% \begin{equation}
% \hat{X}^* = \{\hat{x}_1^*, \hat{x}_2^*, ..., \hat{x}_c^* \}.
% \label{eq:xf}
% \end{equation}
% These images represent the samples that are most semantically aligned with each class and best capture the characteristic attributes of the current category.
\gdd{Through the above auxiliary classifier, we can correct the original prediction probabilities in Eq. \ref{eq:zc} by the zero-shot CLIP as:}
\begin{equation}
\begin{aligned}
{p}_{c}^* &= p_c + \lambda * \hat{p}_c,
\\ \hat{p}_c &= \frac{\text{exp}(\text{sim}(f, F(\hat{x}_c^*)) / \tau)}{\sum_{c^{\prime}=1}^C \text{exp}(\text{sim}(f,F(\hat{x}^*_{c^{\prime}})) / \tau)},
\label{eq:pi}
\end{aligned}
\end{equation}
where $\lambda \geq 0$ serves as a hyper-parameter of these two type predictions. By combining the two predictions, the model's discrimination of the current image contains both semantic and visual perceptual information.
% \subsection{The Overall Training Process}
% \label{ssec:to}
Depending on the discrimination result in Eq. \ref{eq:pi}, we are able to obtain a more comprehensive pseudo label $\tilde{y}^*$ for each sample $x$ as $\tilde{y}^* = \underset{c}{\text{argmax}}{p}_{c}^*$, 
% \begin{equation}
% \tilde{y}_f = \underset{c}{\text{argmax}}p_{fc},
% \label{eq:yf}
% \end{equation}
then, we can use these pseudo-labeled data to optimize the prompt $t$, and the training loss can be expressed as:
\begin{equation}
\underset{t}{\text{min}}\mathcal{L}_{r} = \underset{t}{\text{min}}\mathcal{L}_{ce}(x, \tilde{y}^*).
\label{eq:lr}
\end{equation}

Considering that the synthetic samples generated by stable diffusion in Eq.~\ref{eq:ds} also extend the diversity information of the current category while being labeled counterparts, we participate in the synthetic samples in the training process as well as:
\begin{equation}
\underset{t}{\text{min}}\mathcal{L}_{s} = \underset{t}{\text{min}}\mathcal{L}_{ce}(\hat{x}, y).
\label{eq:ls}
\end{equation}
In conclusion, the training objective of our method can be formally expressed as:
\begin{equation}
\underset{t}{\text{min}}\mathcal{L} = \underset{t}{\text{min}}(\mathcal{L}_{r} + \beta * \mathcal{L}_{s}),
\label{eq:l}
\end{equation}
where $\beta \geq 0$ represents the coefficient of equilibrium between the two loss functions.
After each iteration, the optimized prompt $t$ is sent back to the PLG module and processed through Eq.~\ref{eq:pi} to generate a more accurate pseudo label.
This iterative process facilitates the continuous refinement and optimization of pseudolabels. 
Thus, we not only obtain high-quality pseudo-labeled samples that are classified from semantic and visual perspectives with richer visual perception information but also a diversity of high-quality synthetic samples to aid in training, thus improving the unsupervised prompt learning process.

\subsection{The Overall Training Process}
\label{ssec:to}
% In this subsection, we introduce the overall training process of our method AiR.
% To balance the augmented images’ data diversity and domain consistency, we First Finetune SD with LoRA.
% Then we generate synthetic images $\hat{X}$ through SD and select the sample that best aligns with the semantic information with cosine similarity.
% The selected synthetic images $\hat{X}^*$ serve as image classifier combined with text classifier to discriminate and obtain pseudo-labels $\tilde{y}^*$ for the unlabeled samples.
% Finally, pseudo-labels data $(x, \tilde{y}^*)$ and synthetic data $(\hat{x}, y)$ are used as training samples to compute the loss and iteratively optimize the model parameters.
% The algorithmic flow of our AiR method is as follows:

In this subsection, we outline the overall training process of our method, AiR. 
To balance data diversity and domain consistency in the augmented images, we begin by fine-tuning SD with LoRA. 
Next, synthetic images $\hat{X}$ are generated through SD, and we select the sample best aligned with the semantic information based on cosine similarity. 
The chosen synthetic images $\hat{X}^*$ then act as auxiliary classifiers, in combination with text classifiers, to assign pseudo-labels $\tilde{y}^*$ to the unlabeled samples. 
Finally, the pseudo-labeled data $(x, \tilde{y}^*)$ and synthetic data $(\hat{x}, y)$ serve as training samples to calculate the loss and iteratively optimize the prompt. 
The algorithm of AiR is summarized in the Appendix.
% Algorithm \ref{al:wa}.


% \begin{algorithm}
%     \SetAlgoLined
%     \caption{Workflow about our AiR method for optimizing prompt $t$}
%     \label{al:wa}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     Get pseudo label data $\{x, \tilde{y}\}$ in Eq.\ref{eq:pl} \\
%     Finetune SD with $LoRA$ in Eq.\ref{eq:lora} \\ 
%     Generate synthetic images $\hat{X}$ in Eq.\ref{eq:ds} \\
%     Select high confidence samples $\hat{X}^*$ \\
%     \For{$iter=1,2,3,...$}{
%     Text-image prediction
%     $p_c = \frac{\text{exp}(\text{sim}({f}, {g}_c) / \tau)}{\sum_{c^{\prime}=1}^C \text{exp}(\text{sim}({f}, {g}_{c^{\prime}}) / \tau)}$ \\
%     Image-image prediction
%     $\hat{p}_c = \frac{\text{exp}(\text{sim}({f}, \hat{x}_c^*) / \tau)}{\sum_{c^{\prime}=1}^C \text{exp}(\text{sim}({f}, \hat{x}_{c^{\prime}}^*) / \tau)}$ \\
%     Combine both types of predictions
%     $p_c^* = p_c + \lambda * \hat{p}_c$ \\
%     Pseudo labels $\tilde{y}^* = \underset{c} {\text{argmax}}p_c^*$ \\
%     Real data loss $\underset{t}{\text{min}}\mathcal{L}_{r} = \underset{t}{\text{min}}\mathcal{L}_{ce}(x, \tilde{y}^*)$ \\
%     Synthetic data loss $\underset{t}{\text{min}}\mathcal{L}_{s} = \underset{t}{\text{min}}\mathcal{L}_{ce}(\hat{x}, y)$ \\
%     Total loss $\underset{t}{\text{min}}\mathcal{L} = \underset{t}{\text{min}}(\mathcal{L}_{r} + \beta * \mathcal{L}_{s})$ \\
%     Take gradient descent step on
%     $\nabla \mathcal{L}$ \\
%     Update $t^{iter+1} \leftarrow t^{iter} - \eta \nabla \mathcal{L}$ \\
%     }
% \end{algorithm}

==> CVPR2025_v2/Sections/4_experiments.tex <==
\section{Experiments}
\label{sec:exp}

\inputtable{text_visual_prompt}

\subsection{Benchmark Setting}
\noindent\textbf{Datasets.}
% We conduct a comprehensive evaluation of our method across five classification datasets from diverse domains, including DTD~\cite{cimpoi2014describing}, EuroSAT~\cite{helber2019eurosat}, FGVC~\cite{maji2013fine}, Flowers102~\cite{nilsback2008automated}, and RESISC45~\cite{cheng2017remote}. 
% These datasets encompass a wide range of topics, from generic object, scene, and fine-grained classification, as well as specialized tasks such as texture recognition and satellite imagery analysis.
We conduct a comprehensive evaluation of our method on five diverse classification datasets: DTD \cite{cimpoi2014describing}, EuroSAT \cite{helber2019eurosat}, FGVC \cite{maji2013fine}, Flowers102 \cite{nilsback2008automated}, and RESISC45 \cite{cheng2017remote}. 
These datasets span a wide array of topics, including general object, scene, and fine-grained classification, along with specialized tasks such as texture recognition and satellite imagery analysis.

\noindent\textbf{Learning Paradigms.}
% To thoroughly assess the effectiveness of our method, we explore three common scenarios involving unlabeled data: Unsupervised Learning (UL), Semi-Supervised Learning (SSL), and Transductive Zero-Shot Learning (TRZSL). 
% Detailed explanations of each paradigm and the handling of labeled data can be found in the Appendix.
To comprehensively evaluate the effectiveness of our method, we investigate three common scenarios involving unlabeled data: Unsupervised Learning (UL), Semi-Supervised Learning (SSL), and Transductive Zero-Shot Learning (TRZSL). 
Detailed explanations of each paradigm and our approach to labeled data are provided in the Appendix.

\noindent\textbf{Baselines.} 
% To assess the effectiveness of the training strategies outlined in Sec.\ref{sec:method}, we compare it with CLIP's zero-shot performance with default prompts like `a photo of a CLASS.' 
% Additionally, we benchmark against standard supervised prompt-tuning methods, where only labeled data is used: CoOp~\cite{zhou2022learning} for textual prompts, VPT~\cite{jia2022visual} for visual prompts. 
% Furthermore, we compare our approach, AiR, against three existing unsupervised prompt tuning methods: Few Pseudolabels (FPL)\cite{menghini2023enhancing}, Grow and Refine Iteratively Pseudolabels (GRIP)\cite{menghini2023enhancing}, and CPL~\cite{zhang2024candidate}.
To evaluate the effectiveness of the training strategies outlined in Sec. \ref{sec:method}, we compare ours against CLIP's zero-shot performance using default prompts such as `a photo of a [CLASS]'.
We also benchmark against standard supervised prompt-tuning methods that use only labeled data: CoOp \cite{zhou2022learning} for textual prompts and VPT \cite{jia2022visual} for visual prompts.
Additionally, we compare our approach, AiR, with three existing unsupervised prompt-tuning methods: Few Pseudolabels (FPL) \cite{menghini2023enhancing}, Grow and Refine Iteratively Pseudolabels (GRIP) \cite{menghini2023enhancing}, and CPL \cite{zhang2024candidate}.

\noindent\textbf{Evaluation metrics.}
% We evaluate each method by calculating the test set accuracy, averaging the results across three runs for consistency. 
% For Transductive Zero-Shot Learning (TRZSL), we report the harmonic mean of the accuracies for seen and unseen classes to account for any performance imbalance between the two.
We evaluate each method by calculating test set accuracy and averaging results over three runs for consistency. 
In the case of Transductive Zero-Shot Learning (TRZSL), we report the harmonic mean of accuracies for seen and unseen classes to address potential performance imbalances between them.

\noindent\textbf{Implementation details.}
% In all experiments, across different datasets and learning strategies, we use ViT-B/32 as the vision backbone. 
% For both visual and textual prompt tuning, the prefix size is set to 16. 
% We employ SGD as the optimizer and train for 150 epochs. 
% The learning rate is initially set to 0.0001 for the first 5 warmup epochs, after which it is adjusted to $l$ and decayed using the cosine annealing rule. 
% For textual and visual prompt tuning, $l = 0.1$. 
% In SSL, we use $2$ labeled samples per class to evaluate the impact of pseudo labels when there is minimal labeled data but abundant unlabeled data. 
% The number of iterations is set to $10$. 
% For FPL, the number of pseudo labels per class is fixed at 16 following~\cite{menghini2023enhancing}. 
% For GRIP and CPL, the number of pseudo labels is treated as a hyperparameter that requires tuning following~\cite{zhang2024candidate}.
In all experiments, spanning various datasets and learning strategies, we use ViT-B/32 as the vision backbone. 
We use Stable Diffusion v1-4 as our synthetic data generation model.
For both visual and textual prompt tuning, the prefix size is set to $16$. 
We employ SGD as the optimizer and train for 150 epochs, with an initial learning rate of 0.0001 during the first 5 warmup epochs, after which it is adjusted to $l$ and decayed according to a cosine annealing schedule. 
For both textual and visual prompt tuning, $l$ is set to 0.1.
% In SSL, we use 2 labeled samples per class to evaluate the impact of pseudo-labels in conditions with limited labeled data and abundant unlabeled data.
The number of iterations is set to 10. 
For FPL, the number of pseudo-labels per class is fixed at 16, following \cite{menghini2023enhancing}. 
In GRIP and CPL, the number of pseudo-labels is treated as a tunable hyperparameter following \cite{zhang2024candidate}.

\subsection{Comparison with SOTA Methods}
\label{sec:cw}
% \noindent\textbf{Comparison with prompt Methods.}
% In order to validate the effectiveness of our proposed method AiR, we conducted comparative experiments with three different learning paradigms (SSL,UL,TRAN) on each of the five different datasets and compared them with the contemporary SOTA method.
% We demonstrate the generalization ability of our method by conducting experiments in both the text prompt learning and visual prompt learning frameworks, respectively.

% As shown in Table\ref{tab:tp} and Table\ref{tab:vp}, our approach achieves absolute SOTA results with various datasets and various learning paradigms, and our AiR can be improved by about 2\% on average in the textual prompt learning framework, and about 3\% in the visual prompt learning framework.
% Notably, the enhancement under the visual prompt learning framework is better than that under the textual framework, which we attribute to the fact that visual prompt learning can optimize prompt words that are more adapted to the downstream task images for the large number of samples generated by the SD model, thus enabling the model to capture a wider range of visual perceptual information in the discrimination, and thus enhancing the accuracy of the model's discrimination.
% The overall results also validate that our proposed idea of improving unsupervised prompt learning by augmenting the richness of the discriminant is robust and generalizable, and can perform quite competitively in different scenarios.
To validate the effectiveness of our proposed AiR, we employ CPL~\cite{zhang2024candidate} as a baseline and conduct comparative experiments using three learning paradigms: SSL, UL, and TRZSL on five distinct datasets, benchmarking against contemporary SOTA methods. 
To demonstrate the generalizability of our approach, we evaluate AiR in both text prompt learning and visual prompt learning frameworks.
As shown in Table~\ref{tab:tvp} our approach consistently achieves SOTA results across various datasets and learning paradigms. 
In UL, AiR enhances performance by an average of approximately 2.6\% in text prompt learning and 2.7\% in visual prompt learning. 
In both SSL and TRZSL, AiR achieves performance improvements ranging from 1\% to 3\%. These results indicate that AiR consistently boosts the classification performance of prompt learning models across different learning paradigms. 
This underscores the robustness and generalizability of our approach, demonstrating that augmenting discriminative richness effectively enhances unsupervised prompt learning performance in diverse scenarios.
We also conducted experiments on the large-scale dataset and cross-dataset settings, please refer to the Appendix.
% for more details.
% In UL, AiR improves performance by approximately 2.4\% on average in text prompt learning, and 2.7\% improvement in visual prompt learning.
% In SSL and TRZSL, AiR also improves performance by 1.1\%-4\%.
% This result suggests that our AiR improves the classification performance of prompt learning models regardless of the learning paradigm, and validates the robustness and generalizability of our proposed approach, showing that augmenting discriminative richness can effectively enhance unsupervised prompt learning performance across diverse scenarios.
% by approximately 2.4\% on average in text prompt learning, and 2.7\% improvement in visual prompt learning.
% In the text prompt learning framework, AiR improves performance by approximately 2.4\% on average, while in the visual prompt learning framework, it achieves an average improvement of about 2.7\%. 
% Notably, the visual prompt learning framework yields higher gains, likely because it allows for prompt optimization that is better suited to the downstream task images due to the high diversity of samples generated by the SD model. 
% This enables the model to capture a broader range of visual perceptual information, thereby enhancing its discriminative accuracy.
% Overall, these results 
% validate the robustness and generalizability of our proposed approach, showing that augmenting discriminative richness can effectively enhance unsupervised prompt learning performance across diverse scenarios.

% \inputtable{textual prompts}
% \inputtable{visual_prompt}

\subsection{Ablation Studies}
\noindent\textbf{Effect of Synthetic Prediction and Synthetic Loss.}
% We performed ablation experiments on three different datasets in UL and text prompt paradigm as a way to clearly demonstrate the different gains of each core step in our AiR.
% As shown in Table\ref{tab:abl}, ${P}_{s}$ indicates whether the discriminate results of the synthetic samples are used, and $\mathcal{L}_{s}$ indicates whether the synthetic samples are added to the loss function calculation. 
% To eliminate the influence of other methods, we use GRIP\cite{menghini2023enhancing} as the baseline and report the accuracy performance of the model in each case.
% When using only ${P}_{s}$, the model improves by 1.7\%-5.4\%, which suggests that extending the richness of the discriminant has a quite significant effect on the accuracy improvement of the model.
% Notably, when trained with synthetic samples generated by the SD model, the model still improves by 1.5\%-4.8\%, which suggests that the diversity of the synthetic samples can provide more information to the unsupervised model and help the model to optimize prompt words that are more suitable for downstream tasks. 
% When ${P}_{s}$ and $\mathcal{L}_{s}$ act together in the baseline, the model's performance reaches an optimal state, demonstrating that the discriminative information of enhanced visual perception and the diversity information of the synthetic samples do not overlap the gains to the model, but rather show a superposition effect, further demonstrating the necessity of each step in our AiR model.
We conduct ablation studies on three datasets using the UL and text prompt paradigm to demonstrate the individual contributions of each core component in our AiR method. 
In Table~\ref{tab:abl}, $\hat{p}_{c}$ denotes the inclusion of discriminative results from synthetic samples in Eq. \ref{eq:pi}, $\mathcal{L}_{s}$ indicates whether these synthetic samples contribute to the loss calculation in Eq. \ref{eq:ls}, and $\mathcal{L}_{r}$ indicates whether real samples contribute to the loss calculation in Eq. \ref{eq:lr}. 
To isolate our approach’s impact, we use GRIP \cite{menghini2023enhancing} as the baseline and report model accuracy under each condition. 
When real samples loss function $\mathcal{L}_{r}$ is employed,  using only $\hat{p}_{c}$ yields a 1.7\%-5.4\% improvement, indicating that enriching visual perception discriminative information has a substantial effect on model accuracy. 
Similarly, training with synthetic samples from the SD model together with real samples enhances performance by 1.5\%-4.8\%, showing that sample diversity and fidelity provide valuable information to the unsupervised model, helping it adapt prompts better suited to downstream tasks. 
However, given that our AiR model leverages synthetic samples generated by the SD model for the unsupervised prompt learning task, an important question arises: if only synthetic samples are used for training, is it feasible to fully address the unsupervised learning task? 
As the result shows, the model's performance declines significantly when no real samples are included in the training, for instance, a decrease of $-10.1\%$ in Flowers102 and $-12.3\%$ in RESISC45. 
These results indicate that relying solely on synthetic samples is insufficient for unsupervised learning. Although synthetic samples exhibit sufficient diversity and real-world fidelity, they still cannot fully replace the information provided by real samples.
When $\hat{p}_{c}$, $\mathcal{L}_{s}$, and $\mathcal{L}_{r}$ are combined, the model achieves optimal performance, highlighting that the enhanced visual perception and sample diversity effects are complementary rather than redundant, yielding a compounded improvement. 
We also conducted experiments on the effect of different generation models, please refer to the Appendix for more details.
% These results further validate the necessity of each step in our AiR model.

% \inputtable{ablation}
% \input{Figures/lnl}
% \input{Tables/lora_vs_no_lora}

\noindent\textbf{Effect of LoRA.}
% To verify whether LoRA is necessary for training SD models, we compare the accuracy of SD models with and without LoRA for each dataset in unsupervised paradigm on three different datasets using CPL as the baseline.
% As shown in Fig.\ref{fig:lnl}, the samples generated using LoRA fine-tuned SD give our AiR model a gain of 2\%-3\% higher than the no-use case in the same training environment. 
% It shows that even though SD can generate diverse and fidelity synthetic samples, whether these synthetic samples match the domain of the current dataset is particularly important, and LoRA is indispensable as a part of our AiR model.
To assess the necessity of LoRA for training SD models, we evaluate the accuracy of SD models with and without LoRA on three datasets (RESISC45, Flowers102, EuroSAT, and DTD) in the unsupervised paradigm, with CPL as the baseline. As illustrated in Table \ref{tab:lnl}, synthetic samples generated with LoRA fine-tuning provide our AiR model with a 3\%-8\% accuracy gain compared to the case without LoRA in the same training environment. 
This result highlights that while SD can produce diverse and high-quality synthetic samples, alignment with the dataset’s domain is crucial, making LoRA an indispensable component of our AiR model.
We also conduct ablation experiments on cosine similarity for the sample selected, please refer to the Appendix for more details.


\inputtable{ablation}
\subsection{Exploratory Analysis}

% \noindent\textbf{Sensitivity of $\lambda$}

\noindent\textbf{Sensitivity to the Number of Synthetic Samples.}
% In order to explore the impact of different numbers of synthetic samples on model performance, we experimented with changes in the accuracy of model testing when 30-150 synthetic samples per category were involved in training on the res and eur datasets, respectively.
% As shown in Fig.\ref{fig:nu}, the trend of the line represents the change in model accuracy as the number of synthetic samples increases, and the bubbles represent the number of synthetic samples as a proportion of the number of real samples. We can find that the performance of the model gradually improves as the number of synthetic samples increases, especially when the number improves from 30 to 60, the accuracy of eur improves by 3 points and the accuracy of res improves by 1 point. However, this improvement is not eternal, after the number of synthetic images exceeds 60, the performance improvement of the model becomes slow, and when it exceeds 120, the performance is more regionally smooth. This suggests that synthetic samples do provide richer discriminative information for unsupervised prompt learning, but there is an upper limit to this gain, and in our AiR framework we set the number of synthetic samples to 120 for all learning scenarios.
To investigate the impact of varying numbers of synthetic samples on model performance, we conducted experiments assessing changes in model accuracy with $0$–$150$ synthetic samples per class on the RESISC45 and EuroSAT datasets, respectively.
As shown in Fig.~\ref{fig:nu}, the trend line illustrates how model accuracy shifts with the increasing number of synthetic samples. 
We observe that model performance gradually improves as the number of synthetic samples rises, especially when increasing from $60$ to $90$ samples: EuroSAT accuracy improves by $3\%$, and RESISC45 accuracy by $1\%$. 
However, this improvement is not indefinite; beyond $90$ synthetic images, performance gains slow, and after surpassing $120$ samples, the trend stabilizes. 
This suggests that synthetic samples indeed enrich discriminative information for unsupervised prompt learning and in turn enable noticeable improvement of the model's performance, though there is a limit to this benefit. 
Based on these observations, we set the number of synthetic samples at $120$ across all learning scenarios in our AiR framework.
More experiments about the hyper-parameter $\lambda$ in Eq.~\ref{eq:pi} and $\beta$ in Eq.~\ref{eq:l} are provided in the Appendix.


% \input{Tables/lora_vs_no_lora}


\input{Figures/num}


% \noindent\textbf{Relying Solely on Synthetic Samples.}
% Given that our AiR model leverages synthetic samples generated by the SD model for the unsupervised prompt learning task, an important question arises: if only synthetic samples are used for training, is it feasible to fully address the unsupervised learning task? 
% To explore this, we conduct fully unsupervised experiments on three datasets, using CPL as the baseline and comparing the performance of training with both real and synthetic samples against training with synthetic samples alone.
% As illustrated in Table \ref{tab:on}, in each dataset, the model's performance declines significantly when no real samples are included in the training, for instance, a decrease of $-10.1\%$ in Flowers102, $-4.6\%$ in DTD, and $-12.3\%$ in RESISC45. 
% These results indicate that relying solely on synthetic samples is insufficient for unsupervised learning. Although synthetic samples exhibit sufficient diversity and real-world fidelity, they still cannot fully replace the information provided by real samples.
% We also conducted experiments on the effect of different generative models, please refer to the Appendix for more details.

\input{Tables/lora_vs_no_lora}



\noindent\textbf{Pseudo Label Accuracy.}
% In order to visually demonstrate to what extent the auxiliary classifier constructed with synthetic samples actually improves the pseudo-labeling quality of the model's original text classifier, we take the original `a photo of a' as the text prompt and use the synthetic samples constructed with our AiR model as the reference, and use them on three different datasets to compare the accuracy of pseudo-labeling for top-50 maximum confidence samples.
% As shown in Fig.\ref{fig:pla}, utilizing the proposed synthetic sample-assisted classification of our AiR model, brings at least 3\% enhancement to the original text classification results, and even reaches 6\% on RESISC45, which indicates that augmenting the richness of the discrimination by improving the visual perceptual information can indeed improve the accuracy of the pseudo-labeling, and in turn, enhance the performance of unsupervised prompt learning models.
To demonstrate the extent to which the auxiliary classifier, constructed with synthetic samples, improves the pseudo-labeling quality of the model's original text classifier.
We use the original prompt ``a photo of a" and compare the accuracy of pseudo-labeling for the top 50 maximum confidence samples. 
We employ synthetic samples generated by our AiR model as a reference across three different datasets.
As shown in Fig. \ref{fig:pla}, leveraging synthetic sample-assisted classification within our AiR model results in at least a 3\% improvement in the original text classification accuracy, with a 6\% gain on RESISC45. 
This indicates that augmenting the discriminative richness through enhanced visual perceptual information significantly improves pseudo-labeling accuracy, which in turn boosts the performance of unsupervised prompt learning models.
More experiments about pseudo-label accuracy are provided in the Appendix.

\input{Figures/pla}

\input{Figures/cam}
% \input{Tables/only_psedo_vs_psedo_and_real}

\subsection{Qualitative Analysis}
\noindent\textbf{CAM of Different Discrimination Outcomes.}
To show the effectiveness of synthetic image embeddings intuitively, we use CLIP \cite{radford2021learning} as a baseline and perform CAM (Class Activation Mapping) \cite{zhou2016learning} visualization on two datasets. 
% This enables a clear comparison of the regions of focus for different modalities.
As shown in Fig.~\ref{fig:cam}, we observe that text embeddings sometimes focus on class-irrelevant regions, such as airports in the \emph{Airplane} class, seawater in \emph{Bridge}, and grass in \emph{Blackberry Lily}. 
Additionally, text embeddings may fail to capture all relevant areas, such as part of a \emph{Beach} or a flower petal in \emph{Mexican Aster}. 
When using synthetic samples for discrimination, similar issues arise, but the regions of attention differ. 
For instance, while text embeddings overly focus on airports in \emph{Airplane}, synthetic samples pay less attention to class-relevant regions of the airplane. 
Similarly, text embeddings focus on grass in \emph{Blackberry Lily}, while synthetic samples shift focus to the location of stamens.
This suggests a fundamental difference in the type of information emphasized by different discriminative modalities for the same sample. 
Moreover, when combining the discriminative information from both text and synthetic images, we find that the fused results provide a more complete focus on class-relevant regions while minimizing the influence of class-irrelevant areas. 
For example, the fused attention highlights larger regions of the beach in \emph{Beach} and more complete flowers in \emph{Fire Lily} and \emph{Mexican Aster}.
This result confirms why our AiR method works because when the visual perceptual information embedded in the synthetic samples is used to enhance the richness of the discrimination, it helps the model to focus more on class-relevant regions and suppress activation in class-irrelevant areas, thus resulting in an improvement in model performance.




\input{Figures/tsne}

\noindent\textbf{t-SNE of Different Discrimination Outcomes.}
% In the previous section, we demonstrated the differences in image activation regions by different discriminative methods in terms of CAM, and in this section, we show the state of the spatial distribution of the synthesized image features, the text features, and the sample features from the point of view of t-SNE.
% As shown in Fig.\ref{fig:tsne}, circular dots of different colors represent different classes of images in Flowers102, triangles represent text embeddings corresponding to the color class, squares represent synthetic image embeddings corresponding to the class, and pentagrams represent embeddings after fusing the text embeddings and the synthetic image embeddings in the manner described in Sec.\ref{ssec:lw}.
% From the figure, we can visualize that due to the modality difference, the text embeddings (triangles) collapse to a very small region that is only relatively close to the test samples of the corresponding class, but not in the actual region of the test samples. 
% The synthetic sample embeddings (squares), on the other hand, are directly matched in the data clusters of each class and appear to be more suitable as classifiers than the text embeddings. 
% However, in reality, the different classes of text embeddings are only due to the difference from the image modality, resulting in the use of t-SNE dimensionality reduction in the two-dimensional plane looks too compact, the actual spatial distribution is not necessarily so, so we can not be directly say that the synthetic image embeddings must be more suitable for classification than text embeddings. 
% However, by fusing the two embeddings (pentagrams), it can be clearly seen that the text embeddings have a tendency to move towards the corresponding class of test samples, which indicates that the enhanced discriminative information actually helps the discriminative embeddings calibrate into the corresponding class test samples, thus improving the model's ability to classify different classes.
In the previous section, we demonstrated the differences in image activation regions across various discriminative methods using CAM. 
In this section, we examine the spatial distribution of synthetic image embeddings, text embeddings, and sample embeddings through t-SNE visualization.
As shown in Fig.~\ref{fig:tsne}, circular dots in different colors represent distinct image classes in Flowers102, triangles indicate text embeddings for each class, squares represent synthetic image embeddings, and pentagrams denote the embeddings after fusing text and synthetic image embeddings as outlined in Sec.~\ref{ssec:lw}.
From the figure, it is apparent that due to modality differences, text embeddings (triangles) collapse into a compact region that is only loosely aligned with the corresponding class's test samples, rather than overlapping with them. 
Conversely, the synthetic sample embeddings (squares) align directly with data clusters for each class, appearing more suitable as classifiers compared to the text embeddings.
However, the observed tight clustering of text embeddings in two-dimensional t-SNE space is primarily due to modality discrepancies, which may not reflect their true spatial distribution in higher-dimensional space. 
Thus, we cannot conclude outright that synthetic image embeddings are categorically more suitable for classification.
Nevertheless, by fusing the embeddings (pentagrams), we see a clear tendency for text embeddings to move toward their corresponding test sample classes. 
This shift suggests that augmenting discriminative information effectively calibrates the embeddings, aligning them more closely with the correct test samples and thus improving the model’s classification accuracy across different classes.
More experiments on t-SNE are provided in the appendix.


\noindent\textbf{Fidelity of generated samples $w$ and $w/o$ LoRA.}
% We provide some images generated by the SD model with and without $LoRA$ as a way to more visually demonstrate the necessity of $LoRA$ in our AiR model.
% As shown in Fig.\ref{fig:syn}, the image generated directly without the use of $LoRA$ is roughly similar to the real image, but the difference is very large at a closer look. 
% For example, the shape of flower petals in \textbf{Canterbury Bells}, the viewpoint of an airplane in \textbf{Airplane}, and the appearance of textures in \textbf{Blotchy}, the direct use of the SD model can only roughly generate the corresponding class of images, but can not provide more detailed and more matching information. 
% On the contrary, by using $LoRA$, the shape of the petals in \textbf{Canterbury Bells} is consistent with the real image, the viewpoint of the airplane in \textbf{Airplane} is changed to top view, and the texture in \textbf{Blotchy} is flat and similar. 
% These improvements illustrate that without the use of $LoRA$, synthetic samples that are too different compared to real samples cannot be used as classification embeddings to augment the richness of real discriminative information, demonstrating the necessity of $LoRA$ for our AiR model.
We provide examples of images generated by the SD model with and without LoRA to visually demonstrate the importance of LoRA in our AiR model.
As shown in Fig.~\ref{fig:syn}, images generated without LoRA bear a general resemblance to the real images, yet differ significantly upon closer inspection. 
For instance, the petal shapes in \emph{Canterbury Bells}, the viewpoint in \emph{Airplane}, and the texture details in \emph{Blotchy} reveal substantial mismatches; without LoRA, the SD model can only approximate the overall class, lacking finer, more precise details.
In contrast, with LoRA applied, the generated images exhibit more accuracy in form and detail: the petal shapes in \emph{Canterbury Bells} closely match the real image, the airplane's viewpoint in \emph{Airplane} shifts to a top view, and the texture in \emph{Blotchy} appears smoother and more aligned.
These improvements demonstrate that without LoRA, synthetic samples lack sufficient detailed expression to real samples and cannot effectively serve as classification embeddings to augment discriminative information. 
This underscores the necessity of LoRA in our AiR model.

\input{Figures/syt}


==> CVPR2025_v2/Sections/5_conclusion.tex <==
\section{Conclusion}
% In this paper, we propose a novel auxiliary classification approach AiR.
% The core of our approach is the utilization of the diversity and fidelity of synthetic samples to build an auxiliary classifier that captures richer variations in visual appearance while preserving essential semantics, bridging text-image-pair classification to image-image-pair classification.
% In this way, we can obtain a richer discriminating approach to represent the class comprehensively and thus facilitate classification.
% Our extensive experiments, conducted across five benchmark datasets and three learning paradigms validated the effectiveness of our method. 
% We hope this work provides new thoughts for reducing reliance on labeled data when adapting pre-trained vision-language models like CLIP to new tasks.
In this paper, we introduce AiR, a novel auxiliary classification approach designed to leverage synthetic samples in building an auxiliary classifier. 
In this way, we can capture richer visual variations while preserving core semantics, effectively bridging text-image-pair classification to image-image-pair classification. 
% This method enables a more comprehensive and discriminative representation of classes, facilitating improved classification accuracy. 
Extensive experiments across five benchmark datasets and three learning paradigms validate the effectiveness of our approach. 
We hope this work inspires new approaches to reducing dependence on labeled data when adapting pre-trained vision-language models like CLIP to novel tasks.


==> CVPR2025_v2/Sections/7_Ack.tex <==
\paragraph{Acknowledgements.}
 This work of Dandan Guo was supported by the National Natural Science Foundation of China (NSFC) under Grant 62306125.
 This work of Yi Chang was supported in part by the National Key R\&D Program of China under Grant 2023YFF0905400, in part by the National Natural Science Foundation of China under Grant U2341229. 
 This work of Fan Tang was supported in part by the Beijing Science and Technology Plan Project under no. Z231100005923033, and in part by Beijing Natural Science Foundation under no. L221013.
 

==> CVPR2025_v2/Tables/R1A1.tex <==
\begin{table}[!t]
\centering

\resizebox{.49\textwidth}{!}{
\begin{tabular}{l l l l l l l}
	\toprule
      Method & Flowers102 & FGVCAircraft & RESISC45 &  DTD  & EuroSAT & Average \\ 
      \hline
      % FPL  & 16 & 16 & 16 & 16 & 16 & 16 \\
      CPL/GRIP(Real Image for training prompt)  & 20 (69.8\%) & 60 (16.3\%) & 140 (76.5\%) & 80 (47.1\%) & 2700 (65.8\%) & 600 (64.8\%)\\
      \rowcolor{red!30}
      Ours(Real Image for finetuning DM with LoRA)& 5  (81.8\%) & 10 (25.0\%) & 14  (94.2\%) & 15 (70.1\%) & 1000 (79.5\%) & 244 (79.1\%) \\
      \rowcolor{blue!15}
      Ours(Synthetic Image Learning) & 120 & 120 & 120 & 120 & 120 & 120 \\
      \rowcolor{blue!15}
      Ours(Synthetic Image for ACG) & 1 & 1 & 1 & 1 & 1 & 1\\
      % $\Delta$ & \textcolor{red}{+3.4} & \textcolor{red}{+3.1} & & \textcolor{red}{+4.1} \\
      \bottomrule
\end{tabular}}
\caption{
hh.
% $\Delta$ denotes the magnitude of performance improvement after using LoRA.
%The best results are in \textbf{bold}. 
}
\label{tab:r1a1}
\vspace{-20pt}
\end{table}

==> CVPR2025_v2/Tables/R1A3.tex <==
\begin{table}[!t]
\centering

\resizebox{.35\textwidth}{!}{
\begin{tabular}{c c c c }
\toprule
 Method  & &ImageNet & \\
   & SSL & UL  & TRZSL \\ 
\hline
CPL & 61.6 & 62.8  &  65.3 \\ 
\rowcolor{gray!15}
Ours & \textbf{63.9}  & \textbf{64.9}  &  \textbf{67.2} \\ 
\bottomrule
\end{tabular}
}


\caption{Comparison results of top-1 test accuracy (\%) on ImageNet dataset.
The best results are in \textbf{bold}.
}

\label{tab:r1a3}
% \vspace{-20pt}
\end{table}

==> CVPR2025_v2/Tables/R2A1.tex <==
\begin{table}[!t]
\centering

\resizebox{.45\textwidth}{!}{
\begin{tabular}{c c c c c c}
\toprule
 $\mathcal{L}_{r}$  & $\hat{p}_{c}$ & $\mathcal{L}_{s}$  & RESICS45   & Flowers102 & DTD \\ 
\hline
 \rowcolor{red!30}
$\checkmark$ & &  & 70.6 & 69.8 & 46.0  \\
$\checkmark$   &$\checkmark$  &   & 72.3 & 71.6  & 51.4 \\
\rowcolor{blue!30}
 &  & $\checkmark$ & 58.3 & 59.7 & 41.4 \\
 \rowcolor{red!30}
$\checkmark$ & & $\checkmark$  & 72.9 & 71.3 & 50.8  \\ 
\rowcolor{gray!15}
$\checkmark$ & $\checkmark$  & $\checkmark$ & \textbf{73.6} & \textbf{71.9} & \textbf{52.3} \\ 
\bottomrule
\end{tabular}
}


\caption{hh.
%The best results are in \textbf{bold}.
}

\label{tab:r2a1}
% \vspace{-20pt}
\end{table}

==> CVPR2025_v2/Tables/R3A5.tex <==
\begin{table}[!t]
\centering
\resizebox{.45\textwidth}{!}{
% \setlength{\tabcolsep}{2.2mm}{
\begin{tabular}{l  c | c c c c c}
	\toprule
      Method  & Source  &  & & Target & & \\
       &RESISC45 &Flowers102 &FGVCaircraft &DTD &EuroSAT  & Average\\
    \hline
    CPL & 77.3 & 36.2 & 2.6 & 16.9 & 35.3  & 22.7 \\
    \rowcolor{gray!15}
    Ours &  \textbf{79.9} & \textbf{49.6} & \textbf{6.9} & \textbf{24.3} & \textbf{44.5} & \textbf{31.3} \\ 
    \hline
     &Flowers102  &RESISC45  &FGVCaircraft &DTD &EuroSAT  & Average\\
    \hline
    CPL & 72.9 & 20.4 & 6.3 & 20.9 & 34.7 & 20.5 \\
    \rowcolor{gray!15}
    Ours &  \textbf{74.3} & \textbf{28.4} & \textbf{6.5} & \textbf{29.3} & \textbf{39.9} & \textbf{26.0} \\ 
    \hline
     &DTD  &RESISC45  &FGVCaircraft &Flowers102 &EuroSAT  & Average\\
    \hline
    CPL & 51.9 & 40.8 & 4.4 & 45.7 & 27.5 & 29.6 \\
    \rowcolor{gray!15}
    Ours &  \textbf{55.7} & \textbf{44.3} & \textbf{5.2} & \textbf{47.9} & \textbf{32.5} & \textbf{32.5} \\ 
    \bottomrule
\end{tabular}
}
%}
\caption{
Results in cross-dataset scenarios.
}
% \vspace{-20pt}
\label{tab:r3a5}
% }
\end{table}


==> CVPR2025_v2/Tables/ablation.tex <==
\begin{table}[!t]
\centering

\resizebox{.32\textwidth}{!}{
\begin{tabular}{c c c c c c}
\toprule
 $\mathcal{L}_{r}$  & $\hat{p}_{c}$ & $\mathcal{L}_{s}$  & RESICS45   & Flowers102 & DTD \\ 
\hline
$\checkmark$ & &  & 70.6 & 69.8 & 46.0  \\
 &  & $\checkmark$ & 58.3 & 59.7 & 41.4 \\
$\checkmark$   &$\checkmark$  &   & 72.3 & 71.6  & 51.4 \\ 
$\checkmark$ & & $\checkmark$  & 72.9 & 71.3 & 50.8  \\ 
\rowcolor{gray!15}
$\checkmark$ & $\checkmark$  & $\checkmark$ & \textbf{73.6} & \textbf{71.9} & \textbf{52.3} \\ 
\bottomrule
\end{tabular}
}


\caption{Accuracy scores ($\%$) on RESISC45, Flowers102, and DTD are reported to verify the effects of different strategies.
$\hat{p}_{c}$ represents the auxiliary classifier from synthetic samples, $\mathcal{L}_s$ and $\mathcal{L}_r$ indicate the training loss about the synthetic samples and real samples, respectively.
%The best results are in \textbf{bold}.
}

\label{tab:abl}
\vspace{-20pt}
\end{table}

==> CVPR2025_v2/Tables/cos_selec.tex <==
\begin{table}[!t]
\centering

\resizebox{.45\textwidth}{!}{
\begin{tabular}{l c c c }
	\toprule
      Method & Flowers102  & DTD & EuroSAT \\ 
      \hline
      % Cosine Distance & & & \\
      Euclidean Distance &  54.8 & 51.5 &  73.0 \\
      OT distance & 68.3 & 62.3 & 76.6 \\
      \rowcolor{gray!15}
      Cosine Distance & \textbf{68.3} &  \textbf{62.3} &  \textbf{76.6}  \\
      % \hline
%      Cross-entropy pipeline & 57.7 & 88.6 & 81.6 & 80.5 & 67.7  \\ 
      % Ours & 130.2202 & 4.2388 & 21.00  \\
	\bottomrule
\end{tabular}}
\caption{
Comparison of top-1 test accuracy ($\%$) in unsupervised learning with different similarity metrics: Euclidean Distance, OT distance, and Cosine Distance.
The best results are in \textbf{bold}.
}
\label{tab:cos}
% \vspace{-10pt}
\end{table}

==> CVPR2025_v2/Tables/generation_model.tex <==
\begin{table}[!t]
\centering

\resizebox{.45\textwidth}{!}{
\begin{tabular}{l c c c}
	\toprule
      Method & RESISC45  & EuroSAT & DTD \\ 
      \hline
      % Cosine Distance & & & \\
      Kandinsky2.2 & 77.6 & 69.5  & 54.3 \\
      Dreambooth &  78.3 & 70.8 &  54.8    \\
      \rowcolor{gray!15}
      Stable Diffusion & \textbf{79.9} &  \textbf{71.4} &  \textbf{55.7}  \\
      % \hline
%      Cross-entropy pipeline & 57.7 & 88.6 & 81.6 & 80.5 & 67.7  \\ 
      % Ours & 130.2202 & 4.2388 & 21.00  \\
	\bottomrule
\end{tabular}}
\caption{
Comparison of top-1 test accuracy ($\%$) in unsupervised learning with different generative models: Kandinsky2.2, Dreambooth, and Stable Diffusion.
The best results are in \textbf{bold}.
}
\label{tab:gen}
% \vspace{-10pt}
\end{table}

==> CVPR2025_v2/Tables/lora_vs_no_lora.tex <==
\begin{table}[!t]
\centering

\resizebox{.39\textwidth}{!}{
\begin{tabular}{l l l l l}
	\toprule
      LoRA & RESISC45 & Flowers102 &EuroSAT &  DTD  \\ 
      \hline
      $w/o$  & 76.5 & 66.3 & 66.2   & 51.6 \\
      \rowcolor{gray!15}
      $w$  & \inc{\textbf{79.9}}{3.4}  & \inc{\textbf{74.3}}{8.0} & \inc{\textbf{71.4}}{5.2} & \inc{\textbf{55.7}}{4.1} \\
      % $\Delta$ & \textcolor{red}{+3.4} & \textcolor{red}{+3.1} & & \textcolor{red}{+4.1} \\
      \bottomrule
\end{tabular}}
\caption{Comparison results of top-1 test accuracy ($\%$) on unsupervised learning with or without LoRA fine-tuning.
Note that `w/o' denotes the synthetic sample generated without LoRA.
% $\Delta$ denotes the magnitude of performance improvement after using LoRA.
%The best results are in \textbf{bold}. 
}
\label{tab:lnl}
\vspace{-15pt}
\end{table}

==> CVPR2025_v2/Tables/only_psedo_vs_psedo_and_real.tex <==
\begin{table}[!t]
\centering

\resizebox{.39\textwidth}{!}{
\begin{tabular}{l llll}
	\toprule
      LoRA & RESISC45 & Flowers102 & EuroSAT &  DTD  \\ 
      \hline
      \rowcolor{gray!15}
       $S\&R$ & \textbf{79.9} & \textbf{74.3} &\textbf{69.8} & \textbf{55.7} \\
      $S$  & \incb{67.6}{12.3} & \incb{64.2}{10.1} & & \incb{51.1}{4.6} \\
      % $\Delta$ & \textcolor{green}{-12.3} & \textcolor{green}{-10.1} & \textcolor{green}{-4.6} \\
      \bottomrule
\end{tabular}}
\caption{Comparison of top-1 test accuracy ($\%$) in unsupervised learning, with or without the inclusion of real samples in the loss functions. `$S\&R$' denotes the use of synthetic and real samples, while `$S$' indicates the use of only synthetic samples.
% $\Delta$ denotes the decline's magnitude of performance without using real samples.
%The best results are in \textbf{bold}. 
}
\label{tab:on}
\vspace{-10pt}
\end{table}

==> CVPR2025_v2/Tables/text_visual_prompt.tex <==
\begin{table*}[!t]
\centering

\resizebox{\textwidth}{!}{


\begin{tabular}{ l | c  | c c c c c c c c c  c c c c c c c c c }
	\toprule
        \textcolor{blue}{TP} &   & & RESISC45 & & & FGVCAircraft & &  & Flowers102  & & & EuroSAT & & & DTD &  & & Average  &\\ 
      % \hline
       % & & A  & & & R & & & F & &  & F  & & & E & & & D & \\ 
      \hline
       Method & Year  & SSL & UL & TRZSL & SSL & UL & TRZSL & SSL & UL & TRZSL & SSL & UL & TRZSL & SSL & UL & TRZSL & SSL & UL & TRZSL \\
      \hline
       CLIP\cite{radford2021learning} & 2021  & 54.5 & 54.5 & 54.5 & 17.6 & 17.6  & 17.9 & 63.7 & 63.7 & 63.4 & 32.8 & 32.8 & 30.5 & 43.2 & 43.2 & 43.4 & 42.3 & 42.3 & 41.9 \\
       CoOp\cite{zhou2022learning}  & 2022  & 58.5 & - & 63.4 & 14.9  & - & 21.7 & 76.8 & - & 63.2 &59.5 & - & 49.6 & 37.1 & - & 46.3 & 49.3 & - & 48.8\\
      FPL\cite{menghini2023enhancing}  & 2023  & 68.1 & 63.0 & 72.1  & 20.0 & 16.6  & 17.5 & 75.9 & 65.6 & 80.9 &62.0 & 48.9 & 53.7 & 37.1 & 44.9 & 46.3 & 52.6  &  47.8 & 54.0\\
       GRIP\cite{menghini2023enhancing}  & 2023  & 74.1 & 70.6 & 81.1 & 17.0 & 15.2 & 26.1 & 83.6 & 69.8 & 86.8 & 58.6 & 57.2 & 92.3 & 56.0 & 46.0 & 65.3 & 57.8 & 51.7 & 70.3\\
       CPL\cite{zhang2024candidate} & 2024  & 80.9 & 77.3 & 85.8 & 22.4  & 18.3  & 30.8  & 89.6 & 72.9 & 87.3 &75.4 & 67.2 & 93.7 & 61.2 & 51.9 & 68.0 & 65.9 & 57.5 & 73.1 \\
      \rowcolor{gray!15}
      % \multirow{-6}{*}{\rotatebox[origin=c]{90}{TP}}
      Ours & -  & \textbf{82.5} & \textbf{79.9} & \textbf{87.5} & \textbf{24.2} &\textbf{19.6} & \textbf{33.2} & \textbf{91.2} & \textbf{74.3} & \textbf{92.3} &\textbf{76.4} & \textbf{71.4} & \textbf{93.9} & \textbf{62.2} & \textbf{55.7} & \textbf{69.9} & \textbf{67.3} & \textbf{60.1} & \textbf{75.4} \\
      \hline
      \textcolor{red}{VP} &   & & RESISC45 & & & FGVCAircraft & &  & Flowers102  & & & EuroSAT & & & DTD &  & & Average  &\\ 
      \hline
       CLIP\cite{radford2021learning} & 2021 & 54.5 & 54.5 & 54.5 & 17.6 & 17.6  & 17.9  & 63.7 & 63.7 & 63.4 & 32.8 & 32.8 & 30.5 & 43.2 & 43.2 & 43.4 &42.3  & 42.3 & 41.9 \\
       VPT\cite{jia2022visual} & 2022 & 60.8 & - & 67.1 & 17.7  & - & 26.6 & 63.7 & - & 64.7 & 47.1 & - & 62.2 & 36.4 & - & 44.1 & 45.1 & - & 52.9 \\
       FPL\cite{menghini2023enhancing} & 2023  & 65.1 & 62.2 & 67.8  & 20.1 & 18.2 & 16.2 & 67.0 & 65.5 & 71.9 & 52.4 & 48.7 & 68.6 & 47.6 & 47.6  & 52.4  & 50.4 & 48.4 & 55.3 \\
       GRIP\cite{menghini2023enhancing} & 2023  & 71.2 & 68.4 & 82.1  & 19.4 & 17.5  & 26.4 & 67.9 & 63.0 & 77.1 & 63.4 & 63.6 & 96.9 & 54.5 & 50.5 & 62.7 & 55.2 & 52.6 & 68.4 \\
      CPL\cite{zhang2024candidate} & 2024  & 78.4 & 72.9 & 86.6 & 20.5  & 18.2  & 30.2   & 73.5 & 67.2 & 80.1 &72.0 & 68.9 & 98.3 & 58.7 & 53.4 & 65.3 & 60.6 & 56.1 & 72.1 \\
      \rowcolor{gray!15}
      % \multirow{-6}{*}{\rotatebox[origin=c]{90}{VP}}
        Ours & -  & \textbf{81.1} & \textbf{79.3} & \textbf{87.8} & \textbf{23.7} &\textbf{19.3} & \textbf{31.2} & \textbf{78.5} & \textbf{69.2} & \textbf{81.9} &\textbf{73.5} & \textbf{71.6} & \textbf{98.5} & \textbf{59.6} & \textbf{54.6} & \textbf{66.4} & \textbf{63.2} & \textbf{58.8} & \textbf{73.2} \\

	\bottomrule
\end{tabular}}
%}
\caption{Comparison results of top-1 test accuracy($\%$) on five benchmarks.
\textcolor{blue}{TP} and \textcolor{red}{VP} represent applying text prompts and visual prompts as tuning strategies, respectively.
The average accuracy on all datasets is shown on the right.
The best results are in \textbf{bold}.
}
\label{tab:tvp}
\vspace{-10pt}
% }
\end{table*}

==> CVPR2025_v2/Tables/textual_prompts.tex <==
\begin{table}[!t]
\centering

\resizebox{.49\textwidth}{!}{


\begin{tabular}{l | c c c c c c c c c }
	\toprule
       & & Average  & & & RESISC45 & & & FGVCAircraft & \\ 
      \hline
      Method & SSL & UL & TRZSL & SSL & UL & TRZSL & SSL & UL & TRZSL \\
      \hline
      CLIP & 42.3 & 42.3 & 41.9 & 54.5 & 54.5 & 54.5 & 17.6 & 17.6  & 17.9 \\
      CoOp & 49.3 & - & 48.8 & 58.5 & - & 63.4 & 14.9  & - & 21.7 \\
      FPL & 52.6  &  47.8 & 54.0 & 68.1 & 63.0 & 72.1  & 20.0 & 16.6  & 17.5 \\
      GRIP & 57.8 & 51.7 & 70.3 & 74.1 & 70.6 & 81.1 & 17.0 & 15.2 & 26.1 \\
      CPL & 65.9 & 57.5 & 73.1 & 80.9 & 77.3 & 85.8 & 22.4  & 18.3  & 30.8  \\
      \rowcolor{gray!15}
      Ours & \textbf{67.3} & \textbf{59.9} & \textbf{75.4} & \textbf{82.5} & \textbf{79.9} & \textbf{87.5} & \textbf{24.2} &\textbf{19.6} & \textbf{33.2} \\
      \hline
       & & Flowers102  & & & EuroSAT & & & DTD & \\ 
      \hline
      Method & SSL & UL & TRZSL & SSL & UL & TRZSL & SSL & UL & TRZSL \\
      \hline
      CLIP & 63.7 & 63.7 & 63.4 & 32.8 & 32.8 & 30.54 & 43.2 & 43.2 & 43.4 \\
      CoOp& 76.8 & - & 63.2 &59.51 & - & 49.68 & 37.1 & - & 46.3 \\
      FPL & 75.9 & 65.6 & 80.9 &62.0 & 48.9 & 53.7 & 37.1 & 44.9 & 46.3 \\
      GRIP & 83.6 & 69.8 & 86.8 & 58.6 & 57.2 & 92.3 & 56.0 & 46.0 & 65.3 \\
      CPL & 89.6 & 72.9 & 87.3 &75.4 & 67.2 & 93.7 & 61.2 & 51.9 & 68.0 \\
      \rowcolor{gray!15}
      Ours & \textbf{91.2} & \textbf{74.3} & \textbf{92.3} &\textbf{84.7} & \textbf{69.8} & \textbf{93.9} & \textbf{62.2} & \textbf{55.7} & \textbf{69.9}\\
      % \hline
      
      
      % \hline
%      Cross-entropy pipeline & 57.7 & 88.6 & 81.6 & 80.5 & 67.7  \\ 
      % Ours & 130.2202 & 4.2388 & 21.00  \\
	\bottomrule
\end{tabular}}
%}
\caption{Comparison results of top-1 test accuracy($\%$) on five benchmarks when applying text prompts as tuning strategy.
The average accuracy on all datasets is shown on the left top.
The best results are in \textbf{bold}.
}
\label{tab:tp}
% \vspace{-15pt}
% }
\end{table}

==> CVPR2025_v2/Tables/visual_prompt.tex <==
\begin{table}[!t]
\centering

\resizebox{.49\textwidth}{!}{


\begin{tabular}{l | c c c c c c c c c}
	\toprule
       & & Average  & & & RESISC45 & & & FGVCAircraft & \\ 
      \hline
      Method & SSL & UL & TRZSL & SSL & UL & TRZSL & SSL & UL & TRZSL \\
      \hline
      CLIP &42.3  & 42.3 & 41.9 & 54.5 & 54.5 & 54.5 & 17.6 & 17.6  & 17.9 \\
      VPT & 45.1 & - & 52.9 & 60.8 & - & 67.1 & 17.7  & - & 26.6 \\
      FPL & 50.4 & 48.4 & 55.3 & 65.1 & 62.2 & 67.8  & 20.1 & 18.2 & 16.2  \\
      GRIP & 55.2 & 52.6 & 68.4 & 71.2 & 68.4 & 82.1  & 19.4 & 17.5  & 26.4 \\
      CPL & 60.6 & 56.1 & 72.1 & 78.4 & 72.9 & 86.6 & 20.5  & 18.2  & 30.2  \\
      \rowcolor{gray!15}
      Ours & \textbf{} & \textbf{} & \textbf{} & \textbf{81.1} & \textbf{79.3} & \textbf{87.8} & \textbf{23.7} &\textbf{19.3} & \textbf{} \\
      \hline
       & & Flowers  & & & EuroSAT & & & DTD & \\ 
      \hline
       Method & SSL & UL & TRZSL & SSL & UL & TRZSL & SSL & UL & TRZSL \\
      \hline
      CLIP & 63.7 & 63.7 & 63.4 & 32.8 & 32.8 & 30.5 & 43.2 & 43.2 & 43.4 \\
      VPT & 63.7 & - & 64.7 & 47.1 & - & 62.2 & 36.4 & - & 44.1 \\
      FPL & 67.0 & 65.5 & 71.9 & 52.4 & 48.7 & 68.6 & 47.6 & 47.6  & 52.4 \\
      GRIP & 67.9 & 63.0 & 77.1 & 63.4 & 63.6 & 96.9 & 54.5 & 50.5 & 62.7  \\
      CPL & 73.5 & 67.2 & 80.1 &72.0 & 68.9 & 98.3 & 58.7 & 53.4 & 65.3 \\
      \rowcolor{gray!15}
      Ours & \textbf{78.5} & \textbf{69.2} & \textbf{81.9} &\textbf{80.1} & \textbf{71.6} & \textbf{98.5} & \textbf{59.6} & \textbf{54.6} & \textbf{66.4}\\
      % \hline
      
      
      % \hline
%      Cross-entropy pipeline & 57.7 & 88.6 & 81.6 & 80.5 & 67.7  \\ 
      % Ours & 130.2202 & 4.2388 & 21.00  \\
	\bottomrule
\end{tabular}}
%}
\caption{Comparison results of top-1 test accuracy($\%$) on five benchmarks when applying visual prompts as tuning strategy.
The average accuracy on all datasets is shown on the left top.
The best results are in \textbf{bold}.
}
\label{tab:vp}
% \vspace{-15pt}
% }
\end{table}

==> CVPR2025_v2/preamble.tex <==
%
% --- inline annotations
%
\usepackage{lineno}

\newcommand{\inputsection}[1]{\input{Sections/#1}}
\newcommand{\inputfigure}[1]{\input{Figures/#1}}
\newcommand{\inputtable}[1]{\input{Tables/#1}}

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}

\newcommand{\inc}[2]{$#1^{\color{red}+#2}$}
\newcommand{\incb}[2]{$#1^{{{\color{blue}-#2}}}$}
% \captionsetup[algorithm]{name=Algorithm}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}




==> CVPR2025_v2/sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> CVPR2025_v2/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> CVPR2025_v2/sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> CVPR2025_v2/sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> Figures/beta.tex <==
\begin{figure}
\centering

\includegraphics[width=.9\linewidth]{Images/beta.png}
% \vspace{-5pt}
\caption{
Comparison of top-1 test accuracy ($\%$) of pseudo labels with different hyper-parameters $\beta$.
}
% \vspace{-20pt}
\label{fig:beta}
\end{figure}

==> Figures/lamada.tex <==
\begin{figure}
\centering

\includegraphics[width=.9\linewidth]{Images/lambda.png}
% \vspace{-5pt}
\caption{
Comparison of top-1 test accuracy ($\%$) of pseudo labels with different hyper-parameters $\lambda$. 
% `Ours' denotes the use of our approach AiR, while `CLIP' indicates the use of only CLIP's text encoder.
}
% \vspace{-20pt}
\label{fig:lamada}
\end{figure}

==> Figures/lnl.tex <==
\begin{figure}
\centering

\includegraphics[width=.85\linewidth]{Images/lnl.png}
% \vspace{-5pt}
\caption{
Comparison results of top-1 test accuracy ($\%$) on unsupervised learning with or without LoRA fine-tuning.
Note that `w/o' denotes the synthetic sample generated without LoRA.
}
% \vspace{-5pt}
\label{fig:lnl}
\end{figure}

==> Figures/only.tex <==
\begin{figure}
\centering

\includegraphics[width=.85\linewidth]{Images/only.png}
% \vspace{-5pt}
\caption{
Comparison of top-1 test accuracy ($\%$) in unsupervised learning, with or without the inclusion of real samples in the loss functions. `S$\&$R' denotes the use of both synthetic and real samples for loss calculation, while `S' indicates the use of only synthetic samples.
}
% \vspace{-5pt}
\label{fig:on}
\end{figure}

==> Figures/plaa.tex <==
\begin{figure}
\centering

\includegraphics[width=.9\linewidth]{Images/CPL_VS_OURS.png}
% \vspace{-5pt}
\caption{
Comparison of top-1 test accuracy ($\%$) of pseudo labels during different training iterations.
}
% \vspace{-15pt}
\label{fig:plaa}
\end{figure}

==> Figures/sum.tex <==
\begin{figure}
\centering
\vspace{-15pt}
\includegraphics[width=1\linewidth]{Images/sum_v3.pdf}
% \vspace{-20pt}
% \caption{Additional results.
% }
\vspace{-35pt}
\label{fig:sum}
\end{figure}


% Experiments:(a) for \noindent\textbf{\textit{Major Q1}} \textbf{\textit{\textcolor{red}{vVNT}}} and \noindent\textbf{\textit{Q4}} \textbf{\textit{\textcolor{blue}{Lp4P}}}, (b) for \noindent\textbf{\textit{Q1}} \textbf{\textit{\textcolor{cyan}{7Tnt}}}, (c) for \noindent\textbf{\textit{Q5}} \textbf{\textit{\textcolor{blue}{Lp4P}}} and (d) for \noindent\textbf{\textit{Minor Q3}} \textbf{\textit{\textcolor{red}{vVNT}}}.   

==> Figures/tsnee.tex <==
\begin{figure}
\centering

\includegraphics[width=.9\linewidth]{Images/tsne_v3_res_v2.pdf}
% \vspace{-5pt}
\caption{
Visualization of the spatial distribution of synthetic image, text, and sample embeddings
with t-SNE in RESISC45 dataset.
}
% \vspace{-20pt}
\label{fig:tsres}
\end{figure}

==> Figures/tsneee.tex <==
\begin{figure}
\centering

\includegraphics[width=.9\linewidth]{Images/tsne_v3_dtd_v2.pdf}
% \vspace{-5pt}
\caption{
Visualization of the spatial distribution of synthetic image, text, and sample embeddings
with t-SNE in DTD dataset.
}
% \vspace{-20pt}
\label{fig:tsdtd}
\end{figure}

==> Tables/R1A1.tex <==
\begin{table}[!t]
\centering

\resizebox{.49\textwidth}{!}{
\begin{tabular}{l l l l l l l}
	\toprule
      Method & Flowers102 & FGVCAircraft & RESISC45 &  DTD  & EuroSAT & Average \\ 
      \hline
      % FPL  & 16 & 16 & 16 & 16 & 16 & 16 \\
      CPL/GRIP(Real Image for training prompt)  & 20 (69.8\%) & 60 (16.3\%) & 140 (76.5\%) & 80 (47.1\%) & 2700 (65.8\%) & 600 (64.8\%)\\
      \rowcolor{red!30}
      Ours(Real Image for finetuning DM with LoRA)& 5  (81.8\%) & 10 (25.0\%) & 14  (94.2\%) & 15 (70.1\%) & 1000 (79.5\%) & 244 (79.1\%) \\
      \rowcolor{blue!15}
      Ours(Synthetic Image Learning) & 120 & 120 & 120 & 120 & 120 & 120 \\
      \rowcolor{blue!15}
      Ours(Synthetic Image for ACG) & 1 & 1 & 1 & 1 & 1 & 1\\
      % $\Delta$ & \textcolor{red}{+3.4} & \textcolor{red}{+3.1} & & \textcolor{red}{+4.1} \\
      \bottomrule
\end{tabular}}
\caption{
hh.
% $\Delta$ denotes the magnitude of performance improvement after using LoRA.
%The best results are in \textbf{bold}. 
}
\label{tab:r1a1}
\vspace{-20pt}
\end{table}

==> Tables/R1A3.tex <==
\begin{table}[!t]
\centering

\resizebox{.35\textwidth}{!}{
\begin{tabular}{c c c c }
\toprule
 Method  & &ImageNet & \\
   & SSL & UL  & TRZSL \\ 
\hline
CPL & 61.6 & 62.8  &  65.3 \\ 
\rowcolor{gray!15}
Ours & \textbf{63.9}  & \textbf{64.9}  &  \textbf{67.2} \\ 
\bottomrule
\end{tabular}
}


\caption{Comparison results of top-1 test accuracy (\%) on ImageNet dataset.
The best results are in \textbf{bold}.
}

\label{tab:r1a3}
% \vspace{-20pt}
\end{table}

==> Tables/R2A1.tex <==
\begin{table}[!t]
\centering

\resizebox{.45\textwidth}{!}{
\begin{tabular}{c c c c c c}
\toprule
 $\mathcal{L}_{r}$  & $\hat{p}_{c}$ & $\mathcal{L}_{s}$  & RESICS45   & Flowers102 & DTD \\ 
\hline
 \rowcolor{red!30}
$\checkmark$ & &  & 70.6 & 69.8 & 46.0  \\
$\checkmark$   &$\checkmark$  &   & 72.3 & 71.6  & 51.4 \\
\rowcolor{blue!30}
 &  & $\checkmark$ & 58.3 & 59.7 & 41.4 \\
 \rowcolor{red!30}
$\checkmark$ & & $\checkmark$  & 72.9 & 71.3 & 50.8  \\ 
\rowcolor{gray!15}
$\checkmark$ & $\checkmark$  & $\checkmark$ & \textbf{73.6} & \textbf{71.9} & \textbf{52.3} \\ 
\bottomrule
\end{tabular}
}


\caption{hh.
%The best results are in \textbf{bold}.
}

\label{tab:r2a1}
% \vspace{-20pt}
\end{table}

==> Tables/R3A5.tex <==
\begin{table}[!t]
\centering
\resizebox{.45\textwidth}{!}{
% \setlength{\tabcolsep}{2.2mm}{
\begin{tabular}{l  c | c c c c c}
	\toprule
      Method  & Source  &  & & Target & & \\
       &RESISC45 &Flowers102 &FGVCaircraft &DTD &EuroSAT  & Average\\
    \hline
    CPL & 77.3 & 36.2 & 2.6 & 16.9 & 35.3  & 22.7 \\
    \rowcolor{gray!15}
    Ours &  \textbf{79.9} & \textbf{49.6} & \textbf{6.9} & \textbf{24.3} & \textbf{44.5} & \textbf{31.3} \\ 
    \hline
     &Flowers102  &RESISC45  &FGVCaircraft &DTD &EuroSAT  & Average\\
    \hline
    CPL & 72.9 & 20.4 & 6.3 & 20.9 & 34.7 & 20.5 \\
    \rowcolor{gray!15}
    Ours &  \textbf{74.3} & \textbf{28.4} & \textbf{6.5} & \textbf{29.3} & \textbf{39.9} & \textbf{26.0} \\ 
    \hline
     &DTD  &RESISC45  &FGVCaircraft &Flowers102 &EuroSAT  & Average\\
    \hline
    CPL & 51.9 & 40.8 & 4.4 & 45.7 & 27.5 & 29.6 \\
    \rowcolor{gray!15}
    Ours &  \textbf{55.7} & \textbf{44.3} & \textbf{5.2} & \textbf{47.9} & \textbf{32.5} & \textbf{32.5} \\ 
    \bottomrule
\end{tabular}
}
%}
\caption{
Results in cross-dataset scenarios.
}
% \vspace{-20pt}
\label{tab:r3a5}
% }
\end{table}


==> Tables/cos_selec.tex <==
\begin{table}[!t]
\centering

\resizebox{.45\textwidth}{!}{
\begin{tabular}{l c c c }
	\toprule
      Method & Flowers102  & DTD & EuroSAT \\ 
      \hline
      % Cosine Distance & & & \\
      Euclidean Distance &  54.8 & 51.5 &  73.0 \\
      OT distance & 68.3 & 62.3 & 76.6 \\
      \rowcolor{gray!15}
      Cosine Distance & \textbf{68.3} &  \textbf{62.3} &  \textbf{76.6}  \\
      % \hline
%      Cross-entropy pipeline & 57.7 & 88.6 & 81.6 & 80.5 & 67.7  \\ 
      % Ours & 130.2202 & 4.2388 & 21.00  \\
	\bottomrule
\end{tabular}}
\caption{
Comparison of top-1 test accuracy ($\%$) in unsupervised learning with different similarity metrics: Euclidean Distance, OT distance, and Cosine Distance.
The best results are in \textbf{bold}.
}
\label{tab:cos}
% \vspace{-10pt}
\end{table}

==> Tables/generation_model.tex <==
\begin{table}[!t]
\centering

\resizebox{.45\textwidth}{!}{
\begin{tabular}{l c c c}
	\toprule
      Method & RESISC45  & EuroSAT & DTD \\ 
      \hline
      % Cosine Distance & & & \\
      Kandinsky2.2 & 77.6 & 69.5  & 54.3 \\
      Dreambooth &  78.3 & 70.8 &  54.8    \\
      \rowcolor{gray!15}
      Stable Diffusion & \textbf{79.9} &  \textbf{71.4} &  \textbf{55.7}  \\
      % \hline
%      Cross-entropy pipeline & 57.7 & 88.6 & 81.6 & 80.5 & 67.7  \\ 
      % Ours & 130.2202 & 4.2388 & 21.00  \\
	\bottomrule
\end{tabular}}
\caption{
Comparison of top-1 test accuracy ($\%$) in unsupervised learning with different generative models: Kandinsky2.2, Dreambooth, and Stable Diffusion.
The best results are in \textbf{bold}.
}
\label{tab:gen}
% \vspace{-10pt}
\end{table}

==> Tables/only_psedo_vs_psedo_and_real.tex <==
\begin{table}[!t]
\centering

\resizebox{.39\textwidth}{!}{
\begin{tabular}{l llll}
	\toprule
      LoRA & RESISC45 & Flowers102 & EuroSAT &  DTD  \\ 
      \hline
      \rowcolor{gray!15}
       $S\&R$ & \textbf{79.9} & \textbf{74.3} &\textbf{69.8} & \textbf{55.7} \\
      $S$  & \incb{67.6}{12.3} & \incb{64.2}{10.1} & & \incb{51.1}{4.6} \\
      % $\Delta$ & \textcolor{green}{-12.3} & \textcolor{green}{-10.1} & \textcolor{green}{-4.6} \\
      \bottomrule
\end{tabular}}
\caption{Comparison of top-1 test accuracy ($\%$) in unsupervised learning, with or without the inclusion of real samples in the loss functions. `$S\&R$' denotes the use of synthetic and real samples, while `$S$' indicates the use of only synthetic samples.
% $\Delta$ denotes the decline's magnitude of performance without using real samples.
%The best results are in \textbf{bold}. 
}
\label{tab:on}
\vspace{-10pt}
\end{table}

==> Tables/textual_prompts.tex <==
\begin{table}[!t]
\centering

\resizebox{.49\textwidth}{!}{


\begin{tabular}{l | c c c c c c c c c }
	\toprule
       & & Average  & & & RESISC45 & & & FGVCAircraft & \\ 
      \hline
      Method & SSL & UL & TRZSL & SSL & UL & TRZSL & SSL & UL & TRZSL \\
      \hline
      CLIP & 42.3 & 42.3 & 41.9 & 54.5 & 54.5 & 54.5 & 17.6 & 17.6  & 17.9 \\
      CoOp & 49.3 & - & 48.8 & 58.5 & - & 63.4 & 14.9  & - & 21.7 \\
      FPL & 52.6  &  47.8 & 54.0 & 68.1 & 63.0 & 72.1  & 20.0 & 16.6  & 17.5 \\
      GRIP & 57.8 & 51.7 & 70.3 & 74.1 & 70.6 & 81.1 & 17.0 & 15.2 & 26.1 \\
      CPL & 65.9 & 57.5 & 73.1 & 80.9 & 77.3 & 85.8 & 22.4  & 18.3  & 30.8  \\
      \rowcolor{gray!15}
      Ours & \textbf{67.3} & \textbf{59.9} & \textbf{75.4} & \textbf{82.5} & \textbf{79.9} & \textbf{87.5} & \textbf{24.2} &\textbf{19.6} & \textbf{33.2} \\
      \hline
       & & Flowers102  & & & EuroSAT & & & DTD & \\ 
      \hline
      Method & SSL & UL & TRZSL & SSL & UL & TRZSL & SSL & UL & TRZSL \\
      \hline
      CLIP & 63.7 & 63.7 & 63.4 & 32.8 & 32.8 & 30.54 & 43.2 & 43.2 & 43.4 \\
      CoOp& 76.8 & - & 63.2 &59.51 & - & 49.68 & 37.1 & - & 46.3 \\
      FPL & 75.9 & 65.6 & 80.9 &62.0 & 48.9 & 53.7 & 37.1 & 44.9 & 46.3 \\
      GRIP & 83.6 & 69.8 & 86.8 & 58.6 & 57.2 & 92.3 & 56.0 & 46.0 & 65.3 \\
      CPL & 89.6 & 72.9 & 87.3 &75.4 & 67.2 & 93.7 & 61.2 & 51.9 & 68.0 \\
      \rowcolor{gray!15}
      Ours & \textbf{91.2} & \textbf{74.3} & \textbf{92.3} &\textbf{84.7} & \textbf{69.8} & \textbf{93.9} & \textbf{62.2} & \textbf{55.7} & \textbf{69.9}\\
      % \hline
      
      
      % \hline
%      Cross-entropy pipeline & 57.7 & 88.6 & 81.6 & 80.5 & 67.7  \\ 
      % Ours & 130.2202 & 4.2388 & 21.00  \\
	\bottomrule
\end{tabular}}
%}
\caption{Comparison results of top-1 test accuracy($\%$) on five benchmarks when applying text prompts as tuning strategy.
The average accuracy on all datasets is shown on the left top.
The best results are in \textbf{bold}.
}
\label{tab:tp}
% \vspace{-15pt}
% }
\end{table}

==> Tables/visual_prompt.tex <==
\begin{table}[!t]
\centering

\resizebox{.49\textwidth}{!}{


\begin{tabular}{l | c c c c c c c c c}
	\toprule
       & & Average  & & & RESISC45 & & & FGVCAircraft & \\ 
      \hline
      Method & SSL & UL & TRZSL & SSL & UL & TRZSL & SSL & UL & TRZSL \\
      \hline
      CLIP &42.3  & 42.3 & 41.9 & 54.5 & 54.5 & 54.5 & 17.6 & 17.6  & 17.9 \\
      VPT & 45.1 & - & 52.9 & 60.8 & - & 67.1 & 17.7  & - & 26.6 \\
      FPL & 50.4 & 48.4 & 55.3 & 65.1 & 62.2 & 67.8  & 20.1 & 18.2 & 16.2  \\
      GRIP & 55.2 & 52.6 & 68.4 & 71.2 & 68.4 & 82.1  & 19.4 & 17.5  & 26.4 \\
      CPL & 60.6 & 56.1 & 72.1 & 78.4 & 72.9 & 86.6 & 20.5  & 18.2  & 30.2  \\
      \rowcolor{gray!15}
      Ours & \textbf{} & \textbf{} & \textbf{} & \textbf{81.1} & \textbf{79.3} & \textbf{87.8} & \textbf{23.7} &\textbf{19.3} & \textbf{} \\
      \hline
       & & Flowers  & & & EuroSAT & & & DTD & \\ 
      \hline
       Method & SSL & UL & TRZSL & SSL & UL & TRZSL & SSL & UL & TRZSL \\
      \hline
      CLIP & 63.7 & 63.7 & 63.4 & 32.8 & 32.8 & 30.5 & 43.2 & 43.2 & 43.4 \\
      VPT & 63.7 & - & 64.7 & 47.1 & - & 62.2 & 36.4 & - & 44.1 \\
      FPL & 67.0 & 65.5 & 71.9 & 52.4 & 48.7 & 68.6 & 47.6 & 47.6  & 52.4 \\
      GRIP & 67.9 & 63.0 & 77.1 & 63.4 & 63.6 & 96.9 & 54.5 & 50.5 & 62.7  \\
      CPL & 73.5 & 67.2 & 80.1 &72.0 & 68.9 & 98.3 & 58.7 & 53.4 & 65.3 \\
      \rowcolor{gray!15}
      Ours & \textbf{78.5} & \textbf{69.2} & \textbf{81.9} &\textbf{80.1} & \textbf{71.6} & \textbf{98.5} & \textbf{59.6} & \textbf{54.6} & \textbf{66.4}\\
      % \hline
      
      
      % \hline
%      Cross-entropy pipeline & 57.7 & 88.6 & 81.6 & 80.5 & 67.7  \\ 
      % Ours & 130.2202 & 4.2388 & 21.00  \\
	\bottomrule
\end{tabular}}
%}
\caption{Comparison results of top-1 test accuracy($\%$) on five benchmarks when applying visual prompts as tuning strategy.
The average accuracy on all datasets is shown on the left top.
The best results are in \textbf{bold}.
}
\label{tab:vp}
% \vspace{-15pt}
% }
\end{table}

==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
